SHAPO: Sharpness-Aware Policy Optimization for Safe Exploration

Safe exploration is a prerequisite for deploying reinforcement learning (RL) agents in safety-critical domains. In this paper, we approach safe exploration through the lens of epistemic uncertainty, where the actor's sensitivity to parameter perturbations serves as a practical proxy for regions of high uncertainty. We propose Sharpness-Aware Policy Optimization (SHAPO), a sharpness-aware policy update rule that evaluates gradients at perturbed parameters, making policy updates pessimistic with respect to the actor's epistemic uncertainty. Analytically we show that this adjustment implicitly reweighs policy gradients, amplifying the influence of rare unsafe actions while tempering contributions from already safe ones, thereby biasing learning toward conservative behavior in under-explored regions. Across several continuous-control tasks, our method consistently improves both safety and task performance over existing baselines, significantly expanding their Pareto frontiers.

==> iclr2026/sections/effect_of_actor_sam.tex <==
% ====== Preamble bits you can put in your main preamble ======
% \usepackage{amsmath,amssymb,amsthm,mathtools,bm}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary}
\theoremstyle{remark}
% \newtheorem{remark}{Remark}

% Macros
% \newcommand{\E}{\mathbb{E}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\KL}{\mathrm{KL}}
\newcommand{\grad}{\nabla}
\newcommand{\score}{\phi}
% \newcommand{\Fisher}{F}
\newcommand{\normF}[1]{\left\|#1\right\|_{\Fisher^{-1}}}
\newcommand{\ipF}[2]{\left\langle #1,#2\right\rangle_{\Fisher^{-1}}}
\newcommand{\I}{\mathrm{I}}

\renewcommand{\Fisher}{\mathbf{F}}
\newpage

\section{Effect of Actor SAM w/ epistemic uncertainty}
% ====== Main content starts here ======

\paragraph{Standing notation.}
Let $\pi_\theta(a\mid s)$ be a $C^2$ policy with score $\score_\theta(s,a):=\grad_\theta \log\pi_\theta(a\mid s)$ and Fisher information
$\Fisher(\theta):=\E\big[\score_\theta\score_\theta^\top\big]$ under the data‑generating state–action distribution.
Define the TRPO surrogate in minimization form
\begin{equation}
\label{eq:surrogate}
\ell(\theta) := -\,\E\!\left[\frac{\pi_\theta(a\mid s)}{\pi_{\theta_{\text{old}}}(a\mid s)}\,\hat A(s,a)\right],
\end{equation}
with (possibly biased/noisy) advantage estimate $\hat A$ from a non‑SAM critic.
At $\theta=\theta_{\text{old}}$ one has
\begin{equation}
\label{eq:g-def}
g(\theta) := \grad \ell(\theta) = -\,\E\!\left[\hat A(s,a)\,\score_\theta(s,a)\right].
\end{equation}

\begin{assumption}[Local KL quadratic and frozen metric]
\label{ass:fisher-kl}
For small $\Delta$, $\KL(\pi_\theta\|\pi_{\theta+\Delta})=\tfrac12\,\Delta^\top \Fisher(\theta)\Delta + o(\|\Delta\|^2)$. 
In the SAM inner maximization (defined below) we treat $\Fisher(\theta)$ as fixed w.r.t.\ $\Delta$ (``frozen metric'' at the outer point).
\end{assumption}

\begin{definition}[Actor SAM with a KL ellipsoid]
\label{def:sam}
For radius $\rho>0$, define the robustified loss
\begin{equation}
\label{eq:sam}
\ell_{\mathrm{SAM}}(\theta;\rho) := 
\max_{\Delta:\ \Delta^\top \Fisher(\theta)\Delta \le \rho^2}\ \ell(\theta+\Delta).
\end{equation}
\end{definition}

\begin{lemma}[First‑order SAM $\equiv$ natural‑norm regularization]
\label{lem:first-order}
Suppose $\ell$ is $C^1$ and locally first‑order accurate:
$\ell(\theta+\Delta)=\ell(\theta)+g(\theta)^\top\Delta+o(\|\Delta\|)$.
Under Assumption~\ref{ass:fisher-kl},
\begin{equation}
\label{eq:fo-sam}
\ell_{\mathrm{SAM}}(\theta;\rho)
= \ell(\theta) + \rho\,\normF{g(\theta)} + o(\rho),
\qquad
\normF{v}:=\sqrt{v^\top \Fisher(\theta)^{-1}v}.
\end{equation}
The first‑order adversarial perturbation is
\begin{equation}
\label{eq:delta-star}
\Delta^\star(\theta)
= \rho\,\frac{\Fisher(\theta)^{-1}g(\theta)}{\normF{g(\theta)}} + o(\rho).
\end{equation}
\end{lemma}

\begin{proof}[Proof sketch]
The inner problem is linear in $\Delta$ over an ellipsoid; by Cauchy–Schwarz in the $\Fisher$‑metric,
$\max_{\Delta^\top \Fisher \Delta\le \rho^2} g^\top \Delta = \rho \sqrt{g^\top \Fisher^{-1} g}$,
attained at \eqref{eq:delta-star}.
\end{proof}

\begin{proposition}[Danskin characterization]
\label{prop:danskin}
If the maximizer $\Delta^\star(\theta)$ in \eqref{eq:sam} is unique in a neighborhood and Assumption~\ref{ass:fisher-kl} holds, then
\[
\grad_\theta \ell_{\mathrm{SAM}}(\theta;\rho)=\grad_\theta \ell\!\left(\theta+\Delta^\star(\theta)\right)
\quad\text{(to first order in $\rho$)}.
\]
\end{proposition}

\begin{proof}[Proof sketch]
Danskin’s theorem applies since the feasible set is fixed at $\theta$ by the frozen‑metric approximation.
\end{proof}

\begin{theorem}[Local DRO view in policy space]
\label{thm:dro}
Let $\mathcal{B}_\rho(\theta):=\{\vartheta:\ \KL(\pi_\theta,\pi_\vartheta)\le \tfrac12 \rho^2+o(\rho^2)\}$.
Under Assumption~\ref{ass:fisher-kl} and for small $\rho$,
\[
\ell_{\mathrm{SAM}}(\theta;\rho) \;=\; \max_{\vartheta\in \mathcal{B}_\rho(\theta)}\ \ell(\vartheta) \;+\; o(\rho).
\]
Thus actor‑SAM minimizes the worst‑case surrogate over a local KL ball of indistinguishable policies.
\end{theorem}

\begin{corollary}[Risk‑aversion monotonicity]
\label{cor:monotone-rho}
$\partial_\rho \ell_{\mathrm{SAM}}(\theta;\rho)=\normF{g(\theta)}+o(1)\ge 0$. Larger $\rho$ induces locally more conservative updates.
\end{corollary}

\begin{theorem}[Bayesian credible‑set equivalence (epistemic view)]
\label{thm:bayes}
Let $p(\theta\mid\mathcal{D})\approx \mathcal{N}(\hat\theta,\Sigma_n)$ be the Laplace posterior with
$\Sigma_n^{-1}=\kappa n\,\Fisher(\hat\theta)$ for some scaling $\kappa>0$ and effective sample size $n$.
For credibility level $1-\alpha$, the HPD ellipsoid
\[
\mathcal{C}_{1-\alpha}=\left\{\theta:\ (\theta-\hat\theta)^\top \Sigma_n^{-1} (\theta-\hat\theta)\le \chi^2_{d,1-\alpha}\right\}
\]
coincides (up to the quadratic KL approximation) with $\{\Delta:\ \Delta^\top \Fisher(\hat\theta)\Delta \le \rho^2\}$ where
\begin{equation}
\label{eq:rho-alpha}
\rho^2 = \frac{\chi^2_{d,1-\alpha}}{\kappa n}.
\end{equation}
Hence, to first order,
\[
\ell_{\mathrm{SAM}}(\hat\theta;\rho) \;=\; \max_{\theta\in \mathcal{C}_{1-\alpha}} \ell(\theta) \;+\; o(\rho),
\]
i.e., actor‑SAM is worst‑case optimization over a posterior credible set (epistemic risk aversion). As data grows, $\rho=O(n^{-1/2})$.
\end{theorem}

\begin{proposition}[Dual‑norm (information‑geometry) lens]
\label{prop:dual-norm}
Let $m(\theta):=\E[\hat A\,\score_\theta]$ so that $g=-m$.
Define the dual pairing $\langle u,v\rangle:=u^\top v$ with norms $\|v\|_{\Fisher}:=\sqrt{v^\top \Fisher v}$ and $\|u\|_{\Fisher^{-1}}$.
Then
\begin{equation}
\label{eq:dual}
\normF{m} = \sup_{\|v\|_{\Fisher}\le 1} \E\!\left[\hat A\,\langle \score_\theta, v\rangle\right].
\end{equation}
Penalizing $\normF{m}$ suppresses reliance on score directions that yield large advantage gain \emph{per unit KL}, i.e., poorly identified (epistemic‑sensitive) policy directions.
\end{proposition}

\begin{lemma}[Clean upper bounds]
\label{lem:upper-bounds}
By Cauchy–Schwarz applied to \eqref{eq:dual},
\[
\normF{g}=\normF{m}\ \le\ \sqrt{\E[\hat A^2]}.
\]
Alternatively, Jensen on $m=\E[\hat A\,\score]$ gives
$\normF{m} \le \sqrt{\E[\hat A^2\,\score^\top \Fisher^{-1}\score]}=\sqrt{d\,\E[\hat A^2]}$.
\end{lemma}

\begin{remark}[Effect of critic noise]
If $\hat A=A+\varepsilon$ with $\E[\varepsilon]=0$, both bounds in Lemma~\ref{lem:upper-bounds} inflate with $\E[\varepsilon^2]$, i.e., the SAM penalty grows when the actor gradient is driven by a noisier advantage, yielding stronger epistemic hedging.
\end{remark}

\paragraph{Gaussian specialization (fixed covariance).}
Let $\pi_\theta(\cdot\mid s)=\mathcal{N}(\mu_\theta(s),\Sigma)$ with fixed $\Sigma\succ 0$ and $J_\theta\mu_\theta(s)$ the Jacobian.
Then
\[
\score_\theta(s,a)=J_\theta\mu_\theta(s)^\top \Sigma^{-1}\big(a-\mu_\theta(s)\big),\quad
\Fisher(\theta)=\E\!\left[J_\theta\mu_\theta(s)^\top \Sigma^{-1} J_\theta\mu_\theta(s)\right].
\]
Writing $\psi:=J^\top \Sigma^{-1}(a-\mu)$ and $C:=\E[\psi\psi^\top]=\Fisher(\theta)$,
\begin{equation}
\label{eq:gauss-dual}
\normF{g}=\left\|\E[\hat A\,\psi]\right\|_{C^{-1}}
\ \le\ \sqrt{\E[\hat A^2]}\quad\text{(by Proposition~\ref{prop:dual-norm})}.
\end{equation}
An interpretable spectral bound follows from $\|\psi\|^2=(a-\mu)^\top \Sigma^{-1} J J^\top \Sigma^{-1} (a-\mu)$:
\begin{equation}
\label{eq:spectral-bound}
\normF{g}
\ \le\ 
\sqrt{\E[\hat A^2]}\,\sqrt{\lambda_{\max}(C^{-1})}\,
\sqrt{\E\!\left[(a-\mu)^\top \Sigma^{-1} J J^\top \Sigma^{-1} (a-\mu)\right]}.
\end{equation}
Thus SAM down‑weights policy improvements that hinge on large Mahalanobis deviations in states with large sensitivity $J J^\top$.

\begin{assumption}[Local $F$‑smoothness]
\label{ass:f-smooth}
There exists $\lambda>0$ s.t.\ for $\|\Delta\|_{\Fisher}\le \rho$,
$\big\|\grad \ell(\theta+\Delta)-\grad \ell(\theta)\big\|_{\Fisher^{-1}}
\le \lambda\,\|\Delta\|_{\Fisher}$.
Equivalently, the local Hessian is bounded above by $\lambda \Fisher$ in the PSD order.
\end{assumption}

\begin{theorem}[Robust improvement control]
\label{thm:robust-bound}
Under Assumptions~\ref{ass:fisher-kl} and \ref{ass:f-smooth}, any $\Delta$ with $\Delta^\top \Fisher \Delta\le \rho^2$ satisfies
\[
\ell(\theta+\Delta)
\ \le\
\ell(\theta) + g^\top \Delta + \tfrac{\lambda}{2}\,\Delta^\top \Fisher \Delta
\ \le\
\ell(\theta) + \rho\,\normF{g} + \tfrac{\lambda}{2}\rho^2.
\]
Minimizing $\ell(\theta)+\rho\,\normF{g(\theta)}$ therefore controls the local worst‑case loss up to $O(\rho^2)$ curvature—formalizing risk‑averse behavior.
\end{theorem}

\begin{proposition}[Effect on the TRPO step]
\label{prop:step}
Consider the penalized local model $\min_\Delta\ g^\top \Delta + \tfrac{\beta}{2}\Delta^\top \Fisher \Delta$ with solution
$\Delta_{\mathrm{NG}}=-\beta^{-1}\Fisher^{-1}g$.
Augmenting the objective by $\rho\,\normF{g}$ (per Lemma~\ref{lem:first-order}) yields, to first order,
\[
\Delta_{\mathrm{SAM}}
\ \approx\
-\beta^{-1}\Fisher^{-1}\Big(g + \rho\,\grad \normF{g}\Big),
\]
tilting the natural‑gradient away from score directions that make $\normF{g}$ large (sharp/high‑uncertainty directions).
\end{proposition}

\begin{remark}[Why this targets \emph{epistemic} uncertainty even if the critic is not SAMed]
The inner maximization in \eqref{eq:sam} ranges over policies inside a \emph{local KL credible set} (Theorems~\ref{thm:dro}–\ref{thm:bayes}), i.e., policies indistinguishable given current data.
Hence the resulting penalty depends on the actor’s information geometry (via $\Fisher$) rather than the critic’s learning rule.
Noisy/biasy advantages merely scale the penalty (Lemma~\ref{lem:upper-bounds}), which \emph{increases} epistemic conservatism.
\end{remark}


\section{From Bayes Risk to Distortion/Spectral Risk via SAM}

\paragraph{Setup.}
Let $\theta\in\mathbb{R}^d$ be model parameters, $\mathcal{D}$ a dataset, and let $\Pi(\d\theta)$ denote a (variational) posterior over $\theta$ (e.g., Bayes-by-Backprop Gaussian). Let $\ell(\theta;z)$ be a per-sample loss and
\[
L(\theta)\;\triangleq\;\E_{z\sim\mathcal{Z}}[\ell(\theta;z)]
\]
the population loss. The (parameter-)Bayes risk is
\[
\mathcal{R}_{\mathrm{Bayes}}\;\triangleq\;\E_{\Theta\sim\Pi}\!\left[L(\Theta)\right].
\]
Fix a positive-definite metric matrix $M\succ 0$ (e.g., $M=F(\theta)$ Fisher or $M=\Sigma^{-1}$ inverse posterior covariance), and a radius $\rho>0$. The SAM objective centered at $\bar\theta$ is
\[
\mathcal{R}_{\mathrm{SAM}}(\bar\theta)\;\triangleq\;\E_{z}\!\left[\;\max_{\delta:\ \|\delta\|_{M}\le\rho}\ \ell(\bar\theta+\delta;z)\;\right],
\quad
\|\delta\|_{M}\triangleq\sqrt{\delta^\top M\,\delta}.
\]

\paragraph{Distortion/spectral risk preliminaries.}
For an integrable real random variable $X$, let $q_X(u)$ denote its (left-continuous) quantile function. A \emph{distortion risk measure} is
\[
\rho_g(X)\;=\;\int_{0}^{1} q_X(u)\, \d g(u),
\]
for an increasing $g:[0,1]\!\to\![0,1]$ with $g(0)=0$, $g(1)=1$. If $g$ is absolutely continuous with density $\phi(u)=g'(u)$, this is the \emph{spectral} form
\[
\rho_\phi(X)\;=\;\int_0^1 q_X(u)\,\phi(u)\,\d u,
\qquad
\phi\ge 0,\ \int_0^1 \phi=1, \ \phi\ \text{nondecreasing}.
\]
Examples: CVaR$_\alpha$ has $\phi(u)=\tfrac{1}{1-\alpha}\mathbf{1}\{u\ge \alpha\}$; Wang’s transform has $\phi_\lambda(u)$ induced by $g(u)=\Phi\!\big(\Phi^{-1}(u)+\lambda\big)$.

\subsection{First-order equivalence to a spectral risk}
We link SAM to a spectral risk of the Bayes loss by relating the SAM inner maximizer to a \emph{quantile-dependent} reweighting of $L(\Theta)$ under $\Pi$.

\begin{assumption}[Local smoothness and small radius]
\label{ass:smooth}
(i) $L$ is $C^2$ in a neighborhood of $\bar\theta$. (ii) The SAM radius $\rho$ is small so that a second-order Taylor bound of $\ell(\bar\theta+\delta;z)$ at $\delta=0$ is accurate uniformly in $z$. (iii) The inner maximizer is unique and attained at
\[
\delta^*(\bar\theta,z)\;=\;\rho\,\frac{M^{-1}\nabla_\theta \ell(\bar\theta;z)}{\|\nabla_\theta \ell(\bar\theta;z)\|_{M^{-1}}}
\quad\text{(first-order optimality)},
\]
up to $O(\rho)$ error.
\end{assumption}

Define the \emph{local sensitivity index}
\[
S(\bar\theta;z)\;\triangleq\;\|\nabla_\theta \ell(\bar\theta;z)\|_{M^{-1}}
\quad\text{and}\quad
\overline{S}(\bar\theta)\;\triangleq\;\E_{z}[S(\bar\theta;z)].
\]
Under Assumption~\ref{ass:smooth}, a standard envelope/Taylor argument yields
\[
\max_{\|\delta\|_M\le\rho}\ \ell(\bar\theta+\delta;z)
\;=\;
\ell(\bar\theta;z)\;+\;\rho\,S(\bar\theta;z)\;+\;O(\rho^2).
\]
Hence
\begin{equation}
\label{eq:SAM-expansion}
\mathcal{R}_{\mathrm{SAM}}(\bar\theta)
\;=\;
L(\bar\theta)\;+\;\rho\,\overline{S}(\bar\theta)\;+\;O(\rho^2).
\end{equation}

Now inject \emph{parameter uncertainty.} Regard $\bar\theta$ as a typical draw $\Theta\sim\Pi$ (BBB makes this operational), and define random variables
\[
\mathsf{L}\;\triangleq\;L(\Theta),
\qquad
\mathsf{S}\;\triangleq\;\E_{z}\big[\|\nabla_\theta \ell(\Theta;z)\|_{M^{-1}}\big],
\]
both measurable under $(\Theta\sim\Pi)$. Then taking expectation of \eqref{eq:SAM-expansion} w.r.t.\ $\Theta$ gives
\begin{equation}
\label{eq:Bayes-SAM}
\E_{\Theta}\big[\mathcal{R}_{\mathrm{SAM}}(\Theta)\big]
\;=\;
\E[\mathsf{L}]\;+\;\rho\,\E[\mathsf{S}]\;+\;O(\rho^2).
\end{equation}

\begin{assumption}[Rank consistency]
\label{ass:rank}
There exists a Borel function $h:\mathbb{R}\to[0,\infty)$ such that
$\mathsf{S}=h(\mathsf{L})$ almost surely. Moreover $h$ is nondecreasing.
\end{assumption}

Assumption~\ref{ass:rank} states that, under the posterior, larger losses tend to have larger local sensitivity (empirically true in many overparameterized models and PG objectives where gradient magnitudes correlate with ``hard''/unsafe samples).

\begin{theorem}[SAM equals a spectral (distortion) risk to first order]
\label{thm:main}
Under Assumptions~\ref{ass:smooth} and \ref{ass:rank}, let $q_{\mathsf{L}}$ be the quantile function of $\mathsf{L}$ and define
\[
\phi_\rho(u)\;\triangleq\;\frac{1}{Z_\rho}\Big(1+\rho\,h\big(q_{\mathsf{L}}(u)\big)\Big), 
\qquad 
Z_\rho\;\triangleq\;\int_0^1 \Big(1+\rho\,h(q_{\mathsf{L}}(t))\Big)\,\d t.
\]
Then $\phi_\rho$ is nondecreasing and integrates to $1$. Moreover,
\[
\E_{\Theta}\big[\mathcal{R}_{\mathrm{SAM}}(\Theta)\big]
\;=\;
\int_0^1 q_{\mathsf{L}}(u)\,\phi_\rho(u)\,\d u\;+\;O(\rho^2)
\;=\;
\rho_{g_\rho}(\mathsf{L})\;+\;O(\rho^2),
\]
where $g_\rho(u)=\int_0^u \phi_\rho(t)\,\d t$ is a distortion function. In particular, to first order in $\rho$, SAM optimizes a \emph{distortion/spectral risk} of the Bayes loss that overweights upper quantiles in proportion to their conditional gradient magnitude.
\end{theorem}

\begin{proof}[Proof sketch]
Using \eqref{eq:Bayes-SAM} and $\mathsf{S}=h(\mathsf{L})$, write
$
\E[\mathsf{L}] + \rho \E[h(\mathsf{L})]
= \int_0^1 q_{\mathsf{L}}(u)\,\d u + \rho \int_0^1 h(q_{\mathsf{L}}(u))\,\d u.
$
Define $\phi_\rho$ by normalizing $1+\rho h(q_{\mathsf{L}}(u))$ to integrate to 1; since $h$ is nondecreasing and $q_{\mathsf{L}}$ is increasing, $\phi_\rho$ is nondecreasing. Then
$
\int_0^1 q_{\mathsf{L}}(u)\,\phi_\rho(u)\,\d u
= \E[\mathsf{L}] + \rho \E[h(\mathsf{L})] + O(\rho^2)
$
after expanding $Z_\rho^{-1}=1+O(\rho)$, which matches $\E[\mathcal{R}_{\mathrm{SAM}}(\Theta)]$ up to $O(\rho^2)$.
\end{proof}

\paragraph{Interpretation.}
The weight density $\phi_\rho(u)$ tilts the Bayes risk toward higher loss quantiles in proportion to their \emph{expected local sharpness} $h(q_{\mathsf{L}}(u))$. Thus SAM is (to first order) \emph{equivalent to} optimizing a distortion/spectral risk of the Bayes loss, rather than a plain expectation.

\subsection{Recovering familiar distortions (CVaR, Wang) as special cases}

\begin{corollary}[CVaR-like limit]
If $h(l)\approx c\,\mathbf{1}\{l\ge q_{\mathsf{L}}(\alpha)\}$ for some $\alpha\in(0,1)$ and constant $c>0$, then
$\phi_\rho(u)\propto 1+\rho c\,\mathbf{1}\{u\ge\alpha\}$ and, after normalization,
\[
\rho_{g_\rho}(\mathsf{L})
\;\approx\;
(1-\tilde\alpha)\,\E[\mathsf{L}\,|\,\mathsf{L}\le q_{\mathsf{L}}(\tilde\alpha)]
\;+\;(1-(1-\tilde\alpha))\,\mathrm{CVaR}_{\tilde\alpha}(\mathsf{L}),
\]
with $\tilde\alpha=\alpha+O(\rho)$, i.e., SAM approaches a CVaR-type tail emphasis.
\end{corollary}

\begin{corollary}[Wang-type distortion under elliptical posteriors]
Suppose $\Theta\sim\mathcal{N}(\mu,\Sigma)$ (BBB) and local linearization yields $L(\Theta)\approx a+b^\top(\Theta-\mu)$ with $b\neq 0$. If $M=\Sigma^{-1}$ and $h(l)\propto |l-\E[\mathsf{L}]|$ (gradient magnitude proportional to residual under the linearization), then the induced $\phi_\rho$ is (up to normalization) an \emph{exponentially tilted} function of the Gaussian quantile, which coincides with a Wang-type distortion density $\phi_\lambda$ for some $\lambda=\lambda(\rho,\|b\|)$.
\end{corollary}

\paragraph{Second-order refinement.}
Including the $O(\rho^2)$ term yields
\[
\mathcal{R}_{\mathrm{SAM}}(\bar\theta)
= L(\bar\theta) + \rho\,\overline{S}(\bar\theta)
+ \tfrac{\rho^2}{2}\,\E_z\!\left[\lambda_{\max}\!\big(H_M(\bar\theta;z)\big)\right]
+ O(\rho^3),
\]
where $H_M(\bar\theta;z)=M^{-1/2}\nabla^2_\theta \ell(\bar\theta;z)\,M^{-1/2}$.
Averaging over $\Theta$ injects curvature-dependent tail bias; when $\lambda_{\max}$ grows with loss quantiles, it further steepens the spectral weights toward the upper tail (a distortion-strengthening effect).

\subsection{When does the spectral equivalence hold exactly?}
The first-order \emph{equality} with a spectral risk is exact (up to normalization) whenever $\mathsf{S}$ is \emph{measurable w.r.t.\ the $\sigma$-algebra generated by $\mathsf{L}$}, i.e., Assumption~\ref{ass:rank}. In practice this holds approximately when, under the posterior, higher-loss parameter draws systematically exhibit larger local sharpness (common in overparameterized regimes and PG losses where unsafe/rare events have larger gradients).

\subsection{Design choices for Safe RL}
\begin{itemize}
\item \textbf{Metric $M$.} Taking $M=\Sigma^{-1}$ (posterior precision) ties the SAM ball to parameter uncertainty; $M=F(\theta)$ ties it to information geometry. Both inject uncertainty-aware spectral weights.
\item \textbf{Tuning $\rho$.} Larger $\rho$ strengthens tail weights $\phi_\rho$, increasing risk-aversion w.r.t.\ epistemic uncertainty.
\item \textbf{Actor--critic decomposition.} For PG losses with likelihood ratio $\times$ advantage, the same analysis applies to each factor; empirically, adverse (negative-advantage/low-likelihood) samples correlate with larger $S$, thus SAM upweights their quantiles via $\phi_\rho$.
\end{itemize}

\subsection{Limitations and checks}
\begin{itemize}
\item The rank-consistency Assumption~\ref{ass:rank} can fail if gradient magnitudes are not aligned with loss ranks (e.g., saturated regions). Diagnostics: plot $S$ vs.\ $L$ under posterior sampling; monotone trend supports the assumption.
\item For larger $\rho$, second-order (curvature) terms are non-negligible; the induced risk remains a \emph{convex} law-invariant functional but its density deviates from the first-order $\phi_\rho$.
\item Law-invariance hinges on $S$ depending on $\Theta$ only through $L(\Theta)$; otherwise SAM still defines a valid convex risk functional, but not strictly distortion-type.
\end{itemize}



\section*{Setup and Notation}
Let $\theta\in\mathbb{R}^d$ denote policy (or value) network parameters and let $L(\theta)$ be a differentiable surrogate RL loss (e.g., TRPO/PPO actor loss or critic MSE). 
Assume we have epistemic uncertainty over $\theta$ captured by an approximate posterior $q(\vartheta\mid \mathcal{D})$ (e.g., Laplace or Bayes-by-Backprop), and write $\hat\theta$ for a nominal parameter (MAP/mean).

\paragraph{Bayesian RL objective.}
The Bayes risk is
\[
\mathcal{L}_{\mathrm{Bayes}} \;=\; \mathbb{E}_{\vartheta\sim q}[\,L(\vartheta)\,].
\]

\paragraph{SAM objective.}
Given a (semi)norm $\|\cdot\|_{\mathbf{M}} := \sqrt{(\cdot)^\top \mathbf{M}(\cdot)}$ with $\mathbf{M}\succ 0$ (e.g., $\mathbf{M}=\mathbf{I}$ for Euclidean SAM, or $\mathbf{M}=\mathbf{F}(\hat\theta)$ the Fisher for KL-SAM), the SAM loss at $\hat\theta$ is
\[
\mathcal{L}_{\mathrm{SAM}}(\hat\theta;\rho) \;=\; \max_{\|\delta\|_{\mathbf{M}}\le \rho} \, L(\hat\theta+\delta).
\]

\section*{Local models and credible sets}
Assume a second-order local model around $\hat\theta$:
\[
L(\hat\theta+\delta) \;\approx\; L(\hat\theta)+ g^\top \delta + \tfrac{1}{2}\,\delta^\top \mathbf{H}\,\delta,
\quad g:=\nabla L(\hat\theta),\ \mathbf{H}:=\nabla^2 L(\hat\theta).
\]
Assume a Laplace posterior $q(\vartheta\mid\mathcal{D})\approx \mathcal{N}(\hat\theta,\mathbf{\Sigma})$. 
A $(1-\alpha)$ credible ellipsoid is
\[
\mathcal{C}_\alpha \;:=\; \bigl\{\vartheta:\ (\vartheta-\hat\theta)^\top \mathbf{\Sigma}^{-1}(\vartheta-\hat\theta)\le c_\alpha \bigr\},
\]
where $c_\alpha$ is the $\chi^2_d$ quantile.

\paragraph{Fisher--Laplace alignment.}
For many likelihood-based models, the Laplace covariance aligns with the Fisher:
\[
\mathbf{\Sigma}\ \approx\ \kappa\,\mathbf{F}(\hat\theta)^{-1}\quad\text{for some }\kappa>0.
\]
Then $\mathcal{C}_\alpha=\{\hat\theta+\delta:\ \|\delta\|_{\mathbf{F}} \le \sqrt{\kappa\,c_\alpha}\}$.

\section*{First-order forms (risk-neutral vs. worst-case)}
\begin{lemma}[First-order Bayes expansion]
\label{lem:bayes}
Under the local quadratic model and $\vartheta\sim \mathcal{N}(\hat\theta,\mathbf{\Sigma})$,
\[
\mathbb{E}[L(\vartheta)]\ \approx\ L(\hat\theta) + \tfrac{1}{2}\operatorname{Tr}(\mathbf{H}\mathbf{\Sigma}).
\]
\end{lemma}

\begin{lemma}[First-order SAM value]
\label{lem:sam}
With the same local model,
\[
\max_{\|\delta\|_{\mathbf{M}}\le \rho} L(\hat\theta+\delta) \;\approx\; L(\hat\theta) + \rho\,\|g\|_{\mathbf{M}^{-1}} \;+\; \tfrac{1}{2}\rho^2\,\lambda_{\max}\!\bigl(\mathbf{M}^{-1/2}\mathbf{H}\mathbf{M}^{-1/2}\bigr),
\]
and at first order in $\rho$,
\[
\mathcal{L}_{\mathrm{SAM}}(\hat\theta;\rho) \;\approx\; L(\hat\theta) + \rho\,\|g\|_{\mathbf{M}^{-1}}.
\]
The maximizer direction is $\delta^\star \propto \mathbf{M}^{-1} g$.
\end{lemma}

\begin{proof}[Sketch]
Maximize the linear term $g^\top \delta$ subject to $\delta^\top \mathbf{M}\delta\le \rho^2$ by Cauchy–Schwarz in the $\mathbf{M}$-inner product. Quadratic correction yields the $\lambda_{\max}$ term.
\end{proof}

\section*{Equivalence: SAM as worst-posterior Bayes on a credible set}
\begin{theorem}[KL-SAM is worst-case Bayes over a credible ellipsoid (first order)]
\label{thm:equiv}
Suppose $\mathbf{M}=\mathbf{F}(\hat\theta)$ and $\mathbf{\Sigma}=\kappa\,\mathbf{F}^{-1}(\hat\theta)$. 
Let $\rho>0$ and choose $\alpha$ s.t.
\[
\rho^2 \;=\; \kappa\,c_\alpha.
\]
Then
\[
\max_{\vartheta\in \mathcal{C}_\alpha} L(\vartheta) \;\approx\; \mathcal{L}_{\mathrm{SAM}}(\hat\theta;\rho)
\;\approx\; L(\hat\theta) + \rho\,\|g\|_{\mathbf{F}^{-1}} \quad (\text{first order}).
\]
Equivalently,
\[
\mathcal{L}_{\mathrm{SAM}}(\hat\theta;\rho) \;=\; \sup_{Q:\ \operatorname{supp}(Q)\subseteq \mathcal{C}_\alpha}\ \mathbb{E}_{\vartheta\sim Q}[\,L(\vartheta)\,]
\quad (\text{first order}).
\]
\end{theorem}

\begin{proof}[Proof sketch]
The boundary of $\mathcal{C}_\alpha$ is the ellipsoid $\{\delta:\ \|\delta\|_{\mathbf{F}}=\rho\}$. 
Maximizing the linearized loss over this ellipsoid yields $L(\hat\theta)+\rho\|g\|_{\mathbf{F}^{-1}}$, matching Lemma~\ref{lem:sam} with $\mathbf{M}=\mathbf{F}$. 
Allowing $Q$ supported on $\mathcal{C}_\alpha$ cannot beat the boundary point that aligns with $\mathbf{F}^{-1}g$ at first order, so the supremum of expectations equals the boundary maximum.
\end{proof}

\paragraph{Interpretation.}
Bayes averages across the posterior (Lemma~\ref{lem:bayes}); SAM replaces that average by the \emph{worst} parameter in a high-probability credible set matched by $\rho^2=\kappa c_\alpha$ (Theorem~\ref{thm:equiv}). Hence SAM is a \emph{risk-averse} version of Bayesian RL that optimizes a robust/worst-case Bayes loss within a posterior credible region.

\section*{Distortion/risk-measure viewpoint}
Define the ambiguity set $\mathcal{U}_\rho(\hat\theta):=\{Q:\ \operatorname{supp}(Q)\subseteq \{\theta':\|\theta'-\hat\theta\|_{\mathbf{F}}\le \rho\}\}$. 
The functional
\[
\mathsf{R}_\rho[L] \;:=\; \sup_{Q\in \mathcal{U}_\rho(\hat\theta)} \mathbb{E}_{\vartheta\sim Q}[L(\vartheta)]
\]
is a coherent, convex, \emph{parameter-space} risk measure (monotone, translation equivariant, positive homogeneous, subadditive) and coincides (to first order) with the KL-SAM loss. 
It acts like a “distortion” that upweights adverse directions determined by $\mathbf{F}^{-1}g$ rather than a law-invariant distortion on the \emph{outcome} distribution; i.e., it is a \emph{worst-posterior} distortion in parameter space.

\section*{Bayes vs. SAM, second order}
Including the quadratic term gives
\[
\mathbb{E}_{\vartheta\sim q}[L(\vartheta)] \;\approx\; L(\hat\theta) + \tfrac{1}{2}\operatorname{Tr}(\mathbf{H}\mathbf{\Sigma}),\qquad
\mathcal{L}_{\mathrm{SAM}}(\hat\theta;\rho) \;\approx\; L(\hat\theta) + \rho\|g\|_{\mathbf{F}^{-1}} + \tfrac{1}{2}\rho^2\,\lambda_{\max}(\mathbf{F}^{-1/2}\mathbf{H}\mathbf{F}^{-1/2}).
\]
Thus
\[
\mathcal{L}_{\mathrm{SAM}}(\hat\theta;\rho) - \mathbb{E}[L(\vartheta)] 
\;\approx\; \rho\|g\|_{\mathbf{F}^{-1}} + \tfrac{1}{2}\!\left(\rho^2\,\lambda_{\max}(\mathbf{F}^{-1/2}\mathbf{H}\mathbf{F}^{-1/2}) - \operatorname{Tr}(\mathbf{H}\mathbf{\Sigma})\right),
\]
which is nonnegative for typical choices of $\rho$ tied to the credible radius, making the risk-aversion explicit.

\section*{Mapping \texorpdfstring{$\rho$}{rho} to posterior mass \texorpdfstring{$\alpha$}{alpha}}
Under the Fisher–Laplace alignment, picking a posterior mass level $\alpha$ induces
\[
\rho(\alpha) \;=\; \sqrt{\kappa\,c_\alpha}\,,
\]
so SAM’s trust-region radius directly encodes how conservative (risk-averse) you are w.r.t. posterior uncertainty.

\section*{Actor vs. Critic}
For an actor surrogate $L_{\text{actor}}(\theta)=\mathbb{E}[r_t(\theta)\,\hat A_t]$ (TRPO/PPO), KL-SAM uses $\mathbf{M}=\mathbf{F}_{\text{policy}}$, so the worst-case move is along the natural-gradient direction $\mathbf{F}^{-1}g$. 
For a critic MSE, one uses the critic Fisher/ Gauss–Newton metric. 
Both are worst-posterior variants of their corresponding Bayes risks, just in different parameter spaces.

\section*{Takeaway}
Up to standard local (Laplace/second-order) approximations and with KL geometry, 
\[
\boxed{\ \text{SAM} \;\equiv\; \text{Worst-case Bayes over a posterior credible ellipsoid}\ }
\]
hence SAM is a principled, risk-averse refinement of Bayesian RL that selects (locally) the most adverse parameter within a high-probability set, rather than averaging over the posterior.


==> iclr2026/sections/gaussian_policy_analysis.tex <==

\subsection{Analysis of \MethodName{} on a simple Gaussian policy}

\begin{figure}[t]
    \vspace{-0.5cm}

    \centering
\includegraphics[width=0.9\textwidth]{iclr2026/figs/1d_gaussian_plot.png} 
\vspace{-1em}
\caption{\small{\textit{$1D$ Gaussian policy}: The gradient utilized in SHAPO exhibits a larger amplitude for rare and unsafe actions, while it is comparatively smaller for rare safe actions, compared to the classical gradient.}}
    \label{fig:1dGaussian}
        \vspace{-0.3cm}

\end{figure}

Our proposed approach to update the current policy $\pi_0$ is guided by the gradient $\tilde{g}$ of $\ALoss{\pi_0}(\theta)$ evaluated at $\theta_0+\epsilonSAM$, while classical approaches use the gradient $g$ evaluated at $\theta_0$. Here we study how these two gradients $g$ and $\tilde{g}$ differ in a simplified setting.

We assume that the policy at some state is given by a $1D$ Gaussian policy $\pi(a; \mu,1)=\mathcal{N}(a;\mu,1)$ parametrized by the mean $\mu$ and that the current policy is $\pi_0(a)=\pi(a;0,1)$ specified by $\mu_0=0$. We propose to study the discrepancy between the two gradients $g$ and $\tilde{g}$ with respect to $\mu$ in terms of an observed action $a$ and an advantage value $A$ \revision{under a constraint $\deltaSAM$}. Our utility function $\ALoss{\pi_0}$ and its gradient can now be expressed as:
$$
L(\mu;a,A)=\frac{A}{\pi_0(a)}\pi(a;\mu) \quad \nabla_\mu L(\mu;a,A)=\frac{A}{\pi_0(a)}\nabla_\mu\pi(a;\mu) 
$$ 
The standard gradient $g(a,A)= \nabla_\mu L(\mu;a,A)\vert_{\mu=0}$ and the gradient $\tilde{g}(a,A)=\nabla_\mu L(\mu;a,A)\vert_{\mu=\tilde{\mu}}$ at $\tilde{\mu}=\mu_0 +\epsilonSAM$ are as given in the following Proposition (See Appendix \ref{A:Gaussian} for details).
\begin{proposition}
    Under the $1D$ Gaussian model, we have
    \[
    g(a,A)=aA \quad \text{and} \quad \tilde{g}(a,A)={A}{\Delta}\exp\left(\frac{a^2-\Delta^2}{2}\right) \quad\text{with}\quad \Delta=\begin{cases}
        a-\rho &\text{if $Aa<0$}\\
        a+\rho &\text{otherwise,}
    \end{cases}
    \]
    \revision{where $\rho=\sqrt{2\deltaSAM}$.}
    % where $\Delta=a-\rho$ if $Aa<0$ and $a+\rho$ otherwise.
\end{proposition}
Figure~\ref{fig:1dGaussian}, show plots of the two gradients as functions of the action observed $a$ for two values of advantage ($A=-10$ and $A=10$) with $\rho=0.1$ \revision{(i.e. $\deltaSAM=0.005$)}.

We see that \MethodName{} gradients differ from standard gradients for rare actions $|a|>1$. When the advantage is negative, indicating an unsafe action, we see that \MethodName{}'s gradient is larger compared to the standard gradient. In contrast, for positive advantage \MethodName{}'s gradient is smaller than the standard gradient. The analysis of this simplified setting shows that, under certain conditions, \MethodName{}'s policy update promotes a different treatment of rare actions depending on the sign of the corresponding advantage.
When unsafe, rare actions are taken very seriously and an important update of the policy is promoted. In comparison, \MethodName{} opts for smaller updates when facing safe actions, even when they have large advantage. Overall, this behavior aligns well with our safe exploration objectives and helps explain why our approach favors policies that infrequently incur high costs (cf. Figure~\ref{fig:epcost_tail}).




% We observe that the contribution of a single state-action pair $(s,a)$ towards $\ALoss{\pi_0}$ and the corresponding gradient are given by:
% $$
% \ALoss{\pi_0}(\theta|s,a)=\frac{ \Adv(s,a)}{\pi_0(a|s)} \pi_\theta(a|s) \quad \text{and}\quad \nabla_\theta \ALoss{\pi_0}(\theta|s,a)=\frac{ \Adv(s,a)}{\pi_0(a|s)} \nabla_\theta \pi_\theta(a|s)
% $$
% Each observed state-action pair therefore contributes towards the gradient, to increase or decrease the likelihood of action $a$ depending on the sign of $\Adv(s,a)$ (in a way that is inversely proportional to the likelihood of that action under $\pi_0$).

% We fix an arbitrary state $\bar{s}$ and assume a simple $1D$ Gaussian policy $\pi(a; \mu,1)=\mathcal{N}(a;\mu,1)$ parametrized by the mean $\mu$. We choose the current policy to be $\pi_0(a)=\pi(a;0,1)$ specified by $\mu_0=0$ and write $A$ for the value of the advantage $\Adv(\bar{s},a)$ to study the discrepancy between the two gradients in terms of an observed $a$ and an advantage value $A$. \yann{Our utility function at $\pi_0$ and its gradient can be expressed as:
% $$
% L(\mu;a,A)=\frac{A}{\pi_0(a)}\pi(a;\mu) \quad \nabla_\mu L(\mu;a,A)=\frac{A}{\pi_0(a)}\nabla_\mu\pi(a;\mu) 
% $$ 
% We compare the standard gradient $g(a,A)= \nabla_\mu L(\mu;a,A)\vert_{\mu=0}$ with the gradient $\tilde{g}(a,A)=\nabla_\mu L(\mu;a,A)\vert_{\mu=\tilde{\mu}}$ at $\tilde{\mu}=\mu_0 +\epsilonSAM$.
% }
% \begin{proposition}
%     Under the simple $1D$ Gaussian model, we have
%     \[
%     g(a,A)=aA \quad \text{and} \quad \tilde{g}(a,A)={A}{\Delta}\exp\left(\frac{a^2-\Delta^2}{2}\right) \quad\text{with}\quad \Delta=\begin{cases}
%         a-\rho &\text{if $Aa<0$}\\
%         a+\rho &\text{otherwise.}
%     \end{cases}
%     \]
%     % where $\Delta=a-\rho$ if $Aa<0$ and $a+\rho$ otherwise.
% \end{proposition}
 
%  Figure~\ref{fig:1dGaussian}, show plots of the two gradients as functions of the action observed $a$ for two values of advantage ($A=-10$ and $A=10$) with $\rho=0.1$.


% We see that SHAPO gradients differ from standard gradients for rare actions $|a|>1$. When the advantage is negative, indicating an unsafe action, we see that SHAPO's gradient is larger compared to the standard gradient. In contrast, for positive advantage SHAPO's gradient is smaller than the standard gradient. The analysis of this simplified setting shows that, under certain conditions, SHAPO's policy update promotes a different treatment of rare actions depending on the sign of the corresponding advantage.
% When unsafe, rare actions are taken very seriously and an important update of the policy is promoted. In comparison, SHAPO opts for smaller updates when facing safe actions, even when they have large advantage. Overall, this behavior aligns well with our safe exploration objectives and helps explain why our approach favors policies that infrequently incur high costs (cf. Figure~\ref{fig:epcost_tail}).

% \alert{To the extent that the estimation of the advantage related to rare actions is subject to more uncertainty, SHAPO can be seen as placing more trust in a negative advantage, which signifies risk, rather than in a positive advantage.}




% We observe that the contribution of a single state-action pair $(s,a)$ towards $\ALoss{\pi_0}$ and the corresponding gradient are given by:
% $$
% \ALoss{\pi_0}(\theta|s,a)=\frac{ \Adv(s,a)}{\pi_0(a|s)} \pi_\theta(a|s) \quad \text{and}\quad \nabla_\theta \ALoss{\pi_0}(\theta|s,a)=\frac{ \Adv(s,a)}{\pi_0(a|s)} \nabla_\theta \pi_\theta(a|s)
% $$
% Each observed state-action pair therefore contributes towards the gradient, to increase or decrease the likelihood of action $a$ depending on the sign of $\Adv(s,a)$ (in a way that is inversely proportional to the likelihood of that action under $\pi_0$).

% We fix an arbitrary state $\bar{s}$ and assume a simple $1D$ Gaussian policy $\pi(a; \mu,1)=\mathcal{N}(a;\mu,1)$ parametrized by the mean $\mu$. We choose the current policy to be $\pi_0(a)=\pi(a;0,1)$ specified by $\mu_0=0$ and write $A$ for the value of the advantage $\Adv(\bar{s},a)$ to study the discrepancy between the two gradients in terms of an observed $a$ and an advantage value $A$. \yann{Our utility function at $\pi_0$ and its gradient can be expressed as:
% $$
% L(\mu;a,A)=\frac{A}{\pi_0(a)}\pi(a;\mu) \quad \nabla_\mu L(\mu;a,A)=\frac{A}{\pi_0(a)}\nabla_\mu\pi(a;\mu) 
% $$ 
% We compare the standard gradient $g(a,A)= \nabla_\mu L(\mu;a,A)\vert_{\mu=0}$ with the gradient $\tilde{g}(a,A)=\nabla_\mu L(\mu;a,A)\vert_{\mu=\tilde{\mu}}$ at $\tilde{\mu}=\mu_0 +\epsilonSAM$.
% }
% \begin{proposition}
%     Under the simple $1D$ Gaussian model, we have
%     \[
%     g(a,A)=aA \quad \text{and} \quad \tilde{g}(a,A)={A}{\Delta}\exp\left(\frac{a^2-\Delta^2}{2}\right) \quad\text{with}\quad \Delta=\begin{cases}
%         a-\rho &\text{if $Aa<0$}\\
%         a+\rho &\text{otherwise.}
%     \end{cases}
%     \]
%     % where $\Delta=a-\rho$ if $Aa<0$ and $a+\rho$ otherwise.
% \end{proposition}
 
%  Figure~\ref{fig:1dGaussian}, show plots of the two gradients as functions of the action observed $a$ for two values of advantage ($A=-10$ and $A=10$) with $\rho=0.1$.


==> iclr2026/sections/method.tex <==
\section{Method}
\label{sec:method}

\begin{figure}
    \centering
        \includegraphics[width=\linewidth]{iclr2026/figs/actor_sam_fig.png}
    \caption{Caption}
    \label{fig:placeholder}
\end{figure}




\subsection{Problem Setup: CMDP and Lagrangian Policy Optimization}
We consider a constrained Markov decision process (CMDP) defined by
\((\mathcal{S},\mathcal{A},P,r,c,\gamma)\) with discount factor \(\gamma\in(0,1)\).
A policy \(\pi_\theta(a\mid s)\) is parameterized by \(\theta\in\mathbb{R}^p\).
We denote the (discounted) return and cost
\[
J_r(\theta) \;=\; \mathbb{E}\!\left[\sum_{t=0}^{\infty}\gamma^t\, r(s_t,a_t)\right],
\qquad
J_c(\theta) \;=\; \mathbb{E}\!\left[\sum_{t=0}^{\infty}\gamma^t\, c(s_t,a_t)\right],
\]
where the expectation is under the trajectory distribution induced by \(\pi_\theta\).
The safety requirement is \(J_c(\theta)\le \bar{c}\).

We adopt the standard Lagrangian relaxation with multiplier \(\lambda\ge 0\) and
optimize the surrogate loss to be \emph{minimized}
\begin{equation}
\label{eq:lagrangian-loss}
\mathcal{L}_\lambda(\theta)
\;=\; - J_r(\theta) \;+\; \lambda \,\big(J_c(\theta)-\bar{c}\big).
\end{equation}
In practice, we use on-policy surrogates (e.g., TRPO/PPO) with an average KL trust region \(\delta>0\), but we keep the exposition general and write simply \(\mathcal{L}_\lambda\).

\paragraph{Fisher information and average KL.}
Let \(d^{\pi_\theta}\) denote the discounted state occupancy under \(\pi_\theta\).
Define the (empirical) Fisher information
\begin{equation}
\label{eq:fisher}
F(\theta)\;=\; \mathbb{E}_{s\sim d^{\pi_\theta},\,a\sim \pi_\theta(\cdot\mid s)}
\big[\nabla_\theta \log \pi_\theta(a\mid s)\,\nabla_\theta \log \pi_\theta(a\mid s)^\top\big].
\end{equation}
For small parameter changes \(\Delta\), the average KL divergence satisfies the well-known local approximation
\begin{equation}
\label{eq:kl-local}
\overline{\mathrm{KL}}\!\left(\pi_{\theta+\Delta}\;\middle\|\;\pi_\theta\right)
\;=\;\frac{1}{2}\,\Delta^\top F(\theta)\,\Delta + o(\|\Delta\|^2).
\end{equation}

\subsection{Policy-SAM with a KL Trust Region}
\label{subsec:policy-sam}
Sharpness-Aware Minimization (SAM) typically solves \(\min_\theta \max_{\|\epsilon\|\le \rho} \mathcal{L}(\theta+\epsilon)\).
For policies, a geometry compatible with trust-region methods replaces the Euclidean ball by a \emph{KL ball}:
\begin{equation}
\label{eq:kl-sam}
\min_{\theta}\;\max_{\Delta\;\,:\;\,\overline{\mathrm{KL}}(\pi_{\theta+\Delta}\,\|\,\pi_\theta)\;\le\;\rho}
\;\;\mathcal{L}_\lambda(\theta+\Delta).
\end{equation}
We call \eqref{eq:kl-sam} \emph{KL–SAM}. Using \eqref{eq:kl-local}, the inner set is locally the Fisher ellipsoid
\(\{\Delta:\frac{1}{2}\Delta^\top F(\theta)\Delta \le \rho\}\).

\paragraph{First/second-order local model.}
Let \(g(\theta) := \nabla_\theta \mathcal{L}_\lambda(\theta)\) and \(H(\theta):=\nabla_\theta^2 \mathcal{L}_\lambda(\theta)\).
A second-order expansion gives
\begin{equation}
\label{eq:taylor}
\mathcal{L}_\lambda(\theta+\Delta)\;\approx\;\mathcal{L}_\lambda(\theta) \;+\; g(\theta)^\top \Delta \;+\; \frac{1}{2}\,\Delta^\top H(\theta)\,\Delta.
\end{equation}

\subsection{From KL–SAM to Epistemic Risk Aversion}
\label{subsec:epistemic-link}
Our key observation is that the KL–SAM inner maximization is equivalent, locally,
to robustifying \(\mathcal{L}_\lambda\) against parameter uncertainty with respect to the Fisher metric.
This induces a penalty proportional to the \emph{epistemic standard deviation} of the loss under a Laplace (Gaussian) approximation to the posterior.

\begin{lemma}[Linearized inner maximization over a Fisher ellipsoid]
\label{lem:inner-max-linear}
Under the first-order model \(\mathcal{L}_\lambda(\theta+\Delta)\approx \mathcal{L}_\lambda(\theta)+g^\top \Delta\)
and the constraint \(\tfrac{1}{2}\Delta^\top F\,\Delta\le \rho\),
the inner maximization has the unique optimizer
\[
\Delta^\star \;=\; \sqrt{2\rho}\,\frac{F^{-1}g}{\|g\|_{F^{-1}}}
\quad\text{with value}\quad
\max_{\Delta}\; g^\top \Delta \;=\; \sqrt{2\rho}\,\|g\|_{F^{-1}},
\]
where \(\|g\|_{F^{-1}} := \sqrt{g^\top F^{-1} g}\).
\end{lemma}

\begin{proof}
By Lagrange multipliers or Cauchy--Schwarz in the \(F\)-inner product:
\(
g^\top \Delta = \langle g, \Delta\rangle
= \langle F^{-1}g, F\Delta\rangle
\le \|g\|_{F^{-1}}\,\|\Delta\|_{F},
\)
and the constraint implies \(\|\Delta\|_{F}\le \sqrt{2\rho}\).
Equality holds for \(\Delta\propto F^{-1}g\).
\end{proof}

\begin{theorem}[KL--SAM induces mean--std epistemic risk aversion]
\label{thm:mean-std}
Combining \eqref{eq:taylor} with Lemma~\ref{lem:inner-max-linear},
the KL--SAM objective admits the local expansion
\begin{equation}
\label{eq:sam-mean-std}
\max_{\overline{\mathrm{KL}}\le \rho}\;\mathcal{L}_\lambda(\theta+\Delta)
\;=\; \mathcal{L}_\lambda(\theta) \;+\; \underbrace{\sqrt{2\rho}\,\|g(\theta)\|_{F(\theta)^{-1}}}_{\text{epistemic risk penalty}}
\;+\; \frac{1}{2}\,\Delta^{\star\top} H(\theta)\,\Delta^\star \;+\; o(\rho).
\end{equation}
If we approximate the parameter posterior by \(\theta'\sim\mathcal{N}(\theta,\,F(\theta)^{-1})\),
then \(\mathrm{Var}[\mathcal{L}_\lambda(\theta')]\approx g^\top F^{-1}g\), and hence
\[
\sqrt{2\rho}\,\|g\|_{F^{-1}}\;=\;\sqrt{2\rho}\,\sqrt{\mathrm{Var}[\mathcal{L}_\lambda(\theta')]},
\]
i.e., KL--SAM optimizes a mean--standard-deviation (risk-averse) objective with risk-aversion
coefficient \(\beta(\rho)=\sqrt{2\rho}\).
\end{theorem}

\begin{proof}
Insert \(\Delta^\star\) from Lemma~\ref{lem:inner-max-linear} into \eqref{eq:taylor}
to obtain \(\mathcal{L}_\lambda(\theta)+\sqrt{2\rho}\|g\|_{F^{-1}} + \tfrac{1}{2}\Delta^{\star\top}H\Delta^\star + o(\rho)\).
The variance claim follows by linearization: \(\mathcal{L}_\lambda(\theta')\approx \mathcal{L}_\lambda(\theta)+g^\top(\theta'-\theta)\)
with \(\theta'-\theta\sim\mathcal{N}(0,F^{-1})\).
\end{proof}

\begin{remark}[Curvature correction and a spectral bound]
\label{rem:curvature}
Let \(M(\theta):=F(\theta)^{-1/2}H(\theta)F(\theta)^{-1/2}\).
Then \(\Delta^{\star\top}H\Delta^\star = 2\rho\, u^\top M u\) with \(u:=F^{1/2}\Delta^\star/\sqrt{2\rho}\), \(\|u\|_2=1\),
so \(\frac{1}{2}\Delta^{\star\top}H\Delta^\star \in \big[-\rho\|M\|,\,\rho\|M\|\big]\).
Thus
\begin{equation}
\label{eq:upper-lower}
\mathcal{L}_\lambda(\theta)+\sqrt{2\rho}\|g\|_{F^{-1}} - \rho\|M\|
\;\le\;\max_{\overline{\mathrm{KL}}\le \rho}\mathcal{L}_\lambda(\theta+\Delta)
\;\le\;\mathcal{L}_\lambda(\theta)+\sqrt{2\rho}\|g\|_{F^{-1}} + \rho\|M\|.
\end{equation}
\end{remark}

\paragraph{Connection to credible sets and ``how much'' risk aversion.}
Under the Gaussian posterior \(\theta'-\theta\sim\mathcal{N}(0,F^{-1})\), the credible ellipsoid
\(\{\Delta:\Delta^\top F \Delta \le \tau\}\) has coverage level \(\alpha\) when \(\tau=\chi^2_{p}(\alpha)\).
Comparing with \eqref{eq:kl-local}, the KL ball \(\tfrac{1}{2}\Delta^\top F\Delta\le \rho\)
corresponds to the credible ellipsoid with \(\tau=2\rho\).
Therefore,
\begin{equation}
\label{eq:rho-alpha}
\rho \;=\; \tfrac{1}{2}\,\chi^2_{p}(\alpha)
\qquad\Longrightarrow\qquad
\beta(\rho) \;=\; \sqrt{2\rho}\;=\;\sqrt{\chi^2_{p}(\alpha)}.
\end{equation}
Hence a user-chosen credible level \(\alpha\) induces a \emph{quantified} risk-aversion coefficient \(\beta\).

\subsection{Which Loss is Robustified? Lagrangian vs.\ Cost-Only Variants}
\label{subsec:which-loss}
Equation~\eqref{eq:kl-sam} robustifies the Lagrangian loss \(\mathcal{L}_\lambda\), yielding
the penalty \(\sqrt{2\rho}\|g_\lambda\|_{F^{-1}}\) with \(g_\lambda=\nabla\mathcal{L}_\lambda\).
Two practically useful specializations are:
\begin{align}
\textbf{(Lagrangian-SAM)}\quad
&\max_{\overline{\mathrm{KL}}\le \rho}\, \big[-J_r(\theta+\Delta)+\lambda(J_c(\theta+\Delta)-\bar c)\big]
\;\Rightarrow\; \sqrt{2\rho}\,\|\nabla_\theta\mathcal{L}_\lambda\|_{F^{-1}}.
\\
\textbf{(Cost-SAM)}\quad
&\max_{\overline{\mathrm{KL}}\le \rho}\, J_c(\theta+\Delta)
\;\Rightarrow\; \sqrt{2\rho}\,\|\nabla_\theta J_c(\theta)\|_{F^{-1}},
\end{align}
with gradients taken under the policy's on-policy distribution.
Cost-SAM explicitly prioritizes robustness to cost; Lagrangian-SAM balances reward and cost through \(\lambda\).
Both are special cases of \eqref{eq:kl-sam} and inherit Theorem~\ref{thm:mean-std}.

\subsection{Amount of Risk Aversion Induced by \texorpdfstring{\(\rho\)}{rho}}
\label{subsec:how-much-aversion}
The KL--SAM robust objective near \(\theta\) is
\begin{equation}
\label{eq:risk-premium}
\mathcal{R}_\rho(\theta)
:= \max_{\overline{\mathrm{KL}}\le \rho}\mathcal{L}_\lambda(\theta+\Delta)
\;\approx\; \mathcal{L}_\lambda(\theta)
\;+\; \underbrace{\sqrt{2\rho}\,\sigma_{\text{epi}}(\theta)}_{\text{risk premium}}
\;+\; \underbrace{\frac{1}{2}\Delta^{\star\top}H\Delta^\star}_{\text{curvature}},
\quad
\sigma_{\text{epi}}(\theta):=\|g(\theta)\|_{F(\theta)^{-1}}.
\end{equation}
We can therefore \emph{quantify} the incremental epistemic risk load added by \(\rho\) as
\(\mathrm{RP}(\rho,\theta)\approx \sqrt{2\rho}\,\sigma_{\text{epi}}(\theta) + \mathcal{O}(\rho)\).
Using \eqref{eq:rho-alpha}, a desired credible level \(\alpha\) yields
\(\mathrm{RP}(\alpha,\theta)\approx \sqrt{\chi^2_p(\alpha)}\,\sigma_{\text{epi}}(\theta)\).

\subsection{Algorithm: KL--SAM for TRPO/PPO with Safety}
\label{subsec:algorithm}
We implement KL--SAM in two steps per update (like standard SAM), but with a Fisher/KL geometry:

\begin{enumerate}
\item \textbf{Inner (worst-case) point.}
  Given minibatch trajectories, form the on-policy surrogate for \(\mathcal{L}_\lambda\) and compute
  \(g=\nabla_\theta \mathcal{L}_\lambda(\theta)\).
  Compute the \emph{natural} direction \(v \approx F(\theta)^{-1}g\) using conjugate gradient with Fisher–vector products.
  Set the inner point
  \[
  \theta^{(+)} \;=\; \theta \;+\; \Delta^\star,\qquad
  \Delta^\star \;=\; \sqrt{2\rho}\,\frac{v}{\sqrt{g^\top v}}.
  \]
  (This enforces \(\tfrac{1}{2}\Delta^{\star\top}F\Delta^\star=\rho\).)
\item \textbf{Outer (descent) step.}
  Recompute the surrogate gradient at \(\theta^{(+)}\): \(\tilde{g}=\nabla_\theta \mathcal{L}_\lambda(\theta)\big|_{\theta=\theta^{(+)}}\).
  Update \(\theta\) using your preferred trust-region or clipped-ratio step (TRPO/PPO), with KL constraint \(\delta\).
  (Optionally set \(\rho=\delta\) so the SAM radius matches the trust region.)
\item \textbf{Dual update.}
  Update \(\lambda\) by projected gradient ascent on the constraint violation \(J_c(\theta)-\bar c\) (standard).
\end{enumerate}

% \paragraph{Practical notes.}
% (i) Use the empirical Fisher for \(F\) and a small damping \(\epsilon I\) to ensure numerical stability.
% (ii) Sharing Fisher–vector products with the TRPO/PPO step makes the overhead minimal.
% (iii) For Cost-SAM, compute \(g=\nabla_\theta J_c(\theta)\) in Step~1; for Lagrangian-SAM use \(g=\nabla_\theta\mathcal{L}_\lambda(\theta)\).
% (iv) Choose \(\rho\) either as a fraction of the TRPO KL budget \(\delta\) or via a target credible level \(\alpha\) using \eqref{eq:rho-alpha}.

\subsection{Why This Encodes Epistemic (Not Aleatoric) Aversion}
\label{subsec:epistemic-only}
The penalty \(\|g\|_{F^{-1}}\) depends on parameter uncertainty through \(F^{-1}\), i.e., the local posterior covariance under a Laplace approximation. It scales with how uncertain the model is about \(\theta\) (epistemic) and vanishes as \(F^{-1}\to 0\) (data $\uparrow$). In contrast, aleatoric noise (inherent environment randomness) enters the surrogate through gradient variance but \emph{not} through \(F^{-1}\) in the mean–std penalty, cleanly separating the two.

% \subsection{Summary of Guarantees}
% \label{subsec:guarantees}
    % \begin{itemize}
% \item \textbf{Mean–Std Form (Theorem~\ref{thm:mean-std}).}
%   KL--SAM minimizes a local robust objective equal to
%   \(\mathcal{L}_\lambda(\theta)+\beta(\rho)\,\sigma_{\text{epi}}(\theta)+\mathcal{O}(\rho)\),
%   with \(\beta(\rho)=\sqrt{2\rho}\) and \(\sigma_{\text{epi}}(\theta)=\|g\|_{F^{-1}}\).
% \item \textbf{Credible-Level Calibration (Eq.~\eqref{eq:rho-alpha}).}
%   Picking a posterior credible level \(\alpha\) induces \(\rho=\frac{1}{2}\chi^2_p(\alpha)\) and \(\beta(\rho)=\sqrt{\chi^2_p(\alpha)}\).
% \item \textbf{Curvature Control (Remark~\ref{rem:curvature}).}
%   The curvature term is bounded by \(\pm \rho\|F^{-1/2}HF^{-1/2}\|\), quantifying the second-order approximation error and linking safety to local policy smoothness in the Fisher geometry.
% \end{itemize}



% \section{Method}

% \paragraph{Notation.}
% We adopt the CMDP notation from the Background: a stochastic policy $\pi_\theta(a|s)$ with parameters $\theta \in \mathbb{R}^d$, reward and cost returns $J_r(\pi_\theta)$ and $J_c(\pi_\theta)$, and safety threshold $d>0$.
% We work with the \emph{loss-form} Lagrangian
% \[
% \mathcal{L}(\theta,\lambda) \;=\; -\,J_r(\pi_\theta) \;+\; \lambda\big(J_c(\pi_\theta)-d\big),
% \qquad \lambda \ge 0,
% \]
% so that minimizing $\mathcal{L}$ in $\theta$ (and ascending in $\lambda$) is equivalent to maximizing the standard reward Lagrangian.
% We denote by $\Fisher(\theta)$ the Fisher information matrix (FIM) of $\pi_\theta$,
% \[
% \Fisher(\theta)
% := \mathbb{E}_{s \sim d_{\pi_\theta},\, a \sim \pi_\theta(\cdot|s)}
% \!\big[\,\nabla_\theta \log \pi_\theta(a|s)\,\nabla_\theta \log \pi_\theta(a|s)^\top \big],
% \]
% and use the metric-induced norm $\|x\|_{A}:=\sqrt{x^\top A x}$ for any $A\succ 0$.

% \subsection{Robust Lagrangian via Metric-SAM}
% We bias learning toward parameters whose local neighborhoods keep the safety-augmented objective stable by solving the metric-SAM problem
% \begin{equation}
% \label{eq:metric-sam}
% \min_{\theta}\;\max_{\delta \in \mathbb{R}^d}\ \mathcal{L}(\theta+\delta,\lambda)
% \quad\text{s.t.}\quad 
% \delta^\top \Metric(\theta)\, \delta \;\le\; \rho^2,
% \end{equation}
% where $\Metric(\theta)\succ 0$ is a local metric and $\rho>0$ a radius. 
% We specialize to the \emph{Fisher geometry}, $\Metric(\theta)=\Fisher(\theta)$, which second-order approximates an expected KL trust region:
% \[
% \mathbb{E}_{s\sim d_{\pi_\theta}}\!\big[ D_{\mathrm{KL}}(\pi_\theta(\cdot|s)\,\|\,\pi_{\theta+\delta}(\cdot|s))\big]
% \;=\; \tfrac12\,\delta^\top \Fisher(\theta)\,\delta \;+\; o(\|\delta\|^2).
% \]

% For small $\rho$, linearizing $\mathcal{L}$ gives
% $\mathcal{L}(\theta+\delta,\lambda)\approx \mathcal{L}(\theta,\lambda)+ g^\top \delta$ with $g:=\nabla_\theta \mathcal{L}(\theta,\lambda)$.
% The inner problem in \eqref{eq:metric-sam} then has a closed-form solution.

% \begin{lemma}[Inner maximizer under a quadratic constraint]
% \label{lem:inner}
% For $A\succ 0$ and $g\neq 0$,
% \[
% \max_{\delta:\ \delta^\top A \delta \le \rho^2} \ g^\top \delta
% \;=\; \rho\,\sqrt{g^\top A^{-1} g},
% \qquad
% \delta^\star \;=\; \rho\,\frac{A^{-1} g}{\sqrt{g^\top A^{-1} g}}.
% \]
% \emph{Proof sketch.} By Cauchy–Schwarz in the $A$-inner product.
% \end{lemma}

% With $A=\Metric(\theta)$, the first-order reduction of \eqref{eq:metric-sam} is
% \begin{equation}
% \label{eq:outer-regularized}
% \min_{\theta}\ \underbrace{\mathcal{L}(\theta,\lambda)}_{\text{CMDP loss}}
% \;+\; \rho\,\big\|\nabla_\theta \mathcal{L}(\theta,\lambda)\big\|_{\Metric(\theta)^{-1}}.
% \end{equation}
% In particular, for $\Metric(\theta)=\Fisher(\theta)$ the penalty is the \emph{natural-gradient norm} of the Lagrangian, which drives solutions toward \emph{Fisher-flat} regions where local parameter changes have a small effect on the safety-augmented loss.

% \paragraph{Second-order bound.}
% Including curvature, $\mathcal{L}(\theta+\delta,\lambda)\approx \mathcal{L}(\theta,\lambda)+g^\top\delta+\tfrac12\,\delta^\top H\,\delta$ with $H:=\nabla^2_{\theta}\mathcal{L}(\theta,\lambda)$.
% For any $A\succ0$ and $\|\delta\|_{A}\le\rho$,
% \[
% \sup_{\|\delta\|_{A}\le \rho}\ \tfrac12\,\delta^\top H\,\delta
% \;\le\; \tfrac12\,\rho^2\,\lambda_{\max}\!\big(A^{-1/2} H A^{-1/2}\big),
% \]
% clarifying that metric-SAM also discourages large anisotropic curvature measured in the chosen geometry.

% \subsection{Epistemic Credible-Set View}
% Assume a local Gaussian posterior over policy parameters,
% $\theta' \sim \mathcal{N}(\theta,\Sigma(\theta))$, with covariance proportional to the inverse Fisher, $\Sigma(\theta)=\sigma^2 \Fisher(\theta)^{-1}$ (as in Laplace or natural-gradient Bayesian approximations).
% The $\alpha$-credible ellipsoid is
% \[
% \mathcal{C}_\alpha(\theta)
% := \big\{\theta':\ (\theta'-\theta)^\top \Sigma(\theta)^{-1} (\theta'-\theta) \le \chi^2_{d,\alpha}\big\}.
% \]
% Linearizing $\mathcal{L}$,
% \[
% \sup_{\theta'\in \mathcal{C}_\alpha(\theta)} \mathcal{L}(\theta',\lambda)
% \ \approx\ 
% \mathcal{L}(\theta,\lambda) \;+\; \sqrt{\chi^2_{d,\alpha}}\ \|\nabla_\theta \mathcal{L}(\theta,\lambda)\|_{\Sigma(\theta)}.
% \]
% Identifying $\Sigma(\theta) \propto \Fisher(\theta)^{-1}$ shows that metric-SAM with radius $\rho$ coincides (up to scale) with minimizing the worst case of the linearized loss over a local \emph{epistemic} credible set, with the mapping $\rho \propto \sqrt{\chi^2_{d,\alpha}}$.

% \subsection{Actor Update: TRPO/PPO-Style Metric-SAM}
% We implement metric-SAM by the standard two-step SAM procedure adapted to the Fisher geometry.

% \paragraph{Step 1 (adversarial point).}
% Compute the gradient $g=\nabla_\theta \mathcal{L}(\theta,\lambda)$ from current rollouts.
% Form the natural direction via a Fisher–vector product oracle and conjugate gradient (CG),
% $v \approx \Fisher(\theta)^{-1} g$,
% and set
% \[
% \tilde{\theta} \;=\; \theta \;+\; \delta^\star,
% \qquad
% \delta^\star \;=\; \rho\,\frac{v}{\sqrt{g^\top v}}.
% \]

% \paragraph{Step 2 (update from the clean point).}
% Recompute the policy surrogate at the adversarial point $\tilde{\theta}$ and take a trust-region (TRPO) or clipped (PPO) step \emph{from} $\theta$ using those quantities.
% For TRPO, solve
% \[
% \theta^{+} \;=\; \arg\max_{\theta'}\ 
% \mathbb{E}\!\left[\frac{\pi_{\theta'}(a|s)}{\pi_{\theta}(a|s)}\,
% \big(\hat{A}_r^{\,\tilde{\theta}}(s,a) - \lambda\,\hat{A}_c^{\,\tilde{\theta}}(s,a)\big)\right]
% \quad \text{s.t.}\quad 
% \mathbb{E}\!\left[D_{\mathrm{KL}}(\pi_{\theta}\,\|\,\pi_{\theta'})\right]\le \epsilon,
% \]
% where advantages $\hat{A}_r^{\,\tilde{\theta}},\hat{A}_c^{\,\tilde{\theta}}$ are estimated under $\tilde{\theta}$ (e.g., with GAE), while the step is applied to $\theta$.
% For PPO, replace the constraint by ratio clipping (or a KL penalty) using the same adversarial advantages.

% \subsection{Critic Update with SAM}
% Let $\psi$ denote reward- and cost-critic parameters with loss $\ell_V(\psi)$ (squared TD error or GAE regression).
% Apply Euclidean SAM:
% \[
% \psi_{\mathrm{adv}}
% = \psi + \epsilon\,\frac{\nabla_\psi \ell_V(\psi)}{\|\nabla_\psi \ell_V(\psi)\|_2},
% \qquad
% \psi^{+}
% = \psi - \eta_\psi\, \nabla_\psi \ell_V(\psi_{\mathrm{adv}}).
% \]
% (If desired, a metric variant can be used with an approximate Fisher for the critic.)
% SAM reduces overconfident estimates in uncertain regions, stabilizing targets for the actor in the constrained setting.

% \subsection{Dual Update for the Safety Multiplier}
% We update $\lambda$ by projected stochastic ascent on the dual:
% \[
% \lambda^{+} \;=\; \big[\lambda + \eta_\lambda \big(\widehat{J}_c(\pi_\theta)-d\big)\big]_+.
% \]
% A conservative variant evaluates the cost term with trajectories from the adversarial point $\tilde{\theta}$ to better reflect local exposure to uncertainty.

% \subsection{Choosing the Radius \texorpdfstring{$\rho$}{rho}}
% Under the KL approximation, $D_{\mathrm{KL}}(\pi_\theta\|\pi_{\theta+\delta}) \approx \tfrac12 \delta^\top \Fisher(\theta)\delta \le \epsilon$,
% so setting $\rho^2 = 2\epsilon$ matches a TRPO trust region.
% In the credible-set view, pick $\rho = \kappa \sqrt{\chi^2_{d,\alpha}}$ for a target credibility $\alpha$ (the scale $\kappa$ absorbs the proportionality between $\Sigma$ and $\Fisher^{-1}$).

% \subsection{Computation and Practicalities}
% Relative to a vanilla TRPO/PPO update, metric-SAM adds one extra gradient evaluation (at $\tilde{\theta}$) and one CG solve for $v\approx \Fisher^{-1} g$.
% Empirically, this yields a $\sim\!1.5$–$2\times$ per-update overhead while remaining practical in trust-region implementations that already expose Fisher–vector products.
% To avoid degeneracy when $\|g\|_{\Fisher^{-1}}$ is small, cap $\rho$ and/or add a small damping to the Fisher in CG.

% \paragraph{Safety implication.}
% Because \eqref{eq:outer-regularized} penalizes the natural-gradient norm of the safety-augmented loss, the learned policy is explicitly discouraged from parameters where small (epistemically plausible) changes cause large increases in $\mathcal{L}$. This implements risk aversion with respect to epistemic uncertainty and empirically reduces both the \emph{frequency} and the \emph{variance} of constraint violations during training.








==> iclr2026/sections/method_clean.tex <==
%\section{Risk Aware Local Policy Update}

\section{Sharpness aware policy optimization (\MethodName{})}
\label{sec:method}
In the context of policy optimization, SAM framework~\citep{sam} suggests to look for a policy $\pi$ that maximizes 
\begin{equation}\label{SHAPO_obj}
\min_{\tilde{\pi}\in N(\pi)}\ERLag{\lambda}{\tilde{\pi}} 
\end{equation}
instead of just $\ERLag{\lambda}{\pi}$. 
This shift in objectives can be intuitively justified at high level as follows. We may prefer a policy \(\pi_1\) over \(\pi_2\) even if \(\ERLag{\lambda}{\pi_1} < \ERLag{\lambda}{\pi_2}\) if \(\pi_1\) achieves a higher value for the worst-case objective~\ref{SHAPO_obj}. 
This preference may arise from the understanding that the expected return of policies within the neighborhood \(N(\pi_1)\) can provide a more accurate estimate of the actual performance of \(\pi_1\). This is particularly relevant because our learning problem may not fully encapsulate real-world complexities, such as environmental dynamics or the real-world implementation of our policy. By focusing on the worst-case expected return of nearby policies, we aim to better align our estimates with the true performance outcomes in realistic settings.
%This preference arises from the understanding that the neighborhood \(N(\pi_1)\) may serve as a proxy for certain aspects that our learning problem formulation has not fully captured, such as environmental dynamics or the real-world implementation of our policy.

% In this context, if neighboring policies of \(\pi_2\) yield significantly poorer expected returns, it raises concerns about the effective performance and safety of \(\pi_2\). Such discrepancies suggest that if any elements of the modeled problem are inaccurate, \(\pi_2\) may be more susceptible to failure. Therefore, prioritizing policies like \(\pi_1\) that demonstrate robustness in their neighborhood can enhance our confidence in their performance and safety, even if their expected return is lower in a direct comparison.

% \begin{algorithm}[t]
%     \caption{\MethodName{}$(\theta,\Obj{},F,\deltaSAM)$}
%     \begin{algorithmic}[1]
%         \REQUIRE %Policy parametrization $\pi_\theta$,
%         parameter $\theta$,
%         objective function $\Obj{}$, Fisher matrix $F$, constraint $\deltaSAM$     
%         % \STATE Given the SAM constraint $\deltaSAM$ and the optimization objective $\Obj{\pi_\theta}$
%         \STATE Compute the gradient at $\theta$: $ g \gets \nabla_\theta \Obj{}(\theta)\vert_{\theta} $
%         % \STATE Compute Fisher information matrix: $ F \gets \nabla_\theta \nabla_\theta L_{\pi_\theta}(\theta) $
%         \STATE Compute the perturbation: $\textcolor{red}{\epsilonSAM}=U_F(\textcolor{red}{-}g,\deltaSAM)$%$ \epsilon_{\text{SAM}} \gets F^{-1} g $
%         \STATE Compute the gradient at perturbed parameter: $\textcolor{red}{\tilde{g}} \gets  \nabla_\theta \Obj{} (\theta) \vert_{\theta + \textcolor{red}{\epsilonSAM}} $
%         \STATE Return \MethodName{} gradient $\textcolor{red}{\tilde{g}}$
%     \end{algorithmic}
%     \label{SHAPO}
% \end{algorithm}

\subsection{The policy update}

% Here we describe how we integrate the idea of SAM in the context of  reinforcement learning with local policy update.

As outlined in the background section, our goal is to learn a policy \(\pi\) that maximizes \(\ERLag{\lambda}{\pi}\) by gradually updating the current policy \(\pi_{\theta_0}\). This is achieved by solving the optimization problem \ref{TRPO} under a trust region constraint \(\deltaUp\) and using the gradient \(g = \nabla_\theta \ALoss{\pi_0}(\theta) \big|_{\theta = \theta_0}\). 
We present here our proposed approach, which differs primarily in that it substitutes the direction \(g\) with
%\nabla_\theta L_{\pi_0}(\theta) \big|_{\theta = \theta_0 + \epsilon_{\text{SAM}}}\), 
the gradient \(\tilde{g}\) of $\ALoss{\pi_0}$ computed at $\theta_0+\epsilonSAM$ where $\epsilonSAM$ is a carefully chosen adjustment.

% As described in the background section, to eventually learn a policy $\pi$ that maximizes $\ERLag{\lambda}{\pi}$, we gradually update the current policy $\pi_{\theta_0}$ by solving the optimization problem \ref{TRPO} for a trust region constraint $\delta$ and gradient $g=\nabla_\theta L_{\pi_0}(\theta) \vert_{\theta={\theta_0}}$. We now describe our proposed approach that differs only in that it replaces $g$ with a gradient $\tilde{g}=\nabla_\theta L_{\pi_0}(\theta) \vert_{\theta={\theta_0+\epsilonSAM}}$ for a well chosen adjustment $\epsilonSAM$

Given the current policy $\pi_0$, we now outline our proposed method for updating it within the framework of SAM.
 We have at our disposal the utility function $\ALoss{\pi_0}(\theta)$ which estimates the relative improvement (or deterioration) of nearby policies $\pi_\theta$. Our first step therefore consists of solving the minimization problem
\begin{equation}\label{InnerMinAbstract}
\min_{\tilde{\pi}\in N(\pi_0)}\ALoss{\pi_0}({\tilde{\pi}}).    
\end{equation}
We note that choosing an isotropic Euclidean neighborhood in parameter space for $ N(\pi_0) $ presents certain challenges. A small distance in parameter space ($ \|\theta - \theta_0\|_2$ small) does not necessarily guarantee that $ \pi_\theta $ is similar to $ \pi_0 $ in terms of $ \DKLmax $. Consequently, when $ \ALoss{\pi_0}(\theta) < 0 $, it does not ensure that $ \ERLag{\lambda}{\pi_\theta} < \ERLag{\lambda}{\pi_0} $. In contrast, while selecting a neighborhood of distributionally similar policies better reflects the underlying geometry of the statistical manifold of the parameters~\citep{kim2022fisher}, it also contributes to ensure the validity of utility function $\ALoss{\pi_0}$ in virtue of Theorem~\ref{DeviationBound}.

Consequently, to identify a policy $ \tilde{\pi} $ that is distributionally close to $ \pi_{0} $ but performs worse than $ \pi_{0} $, we propose to formulate the inner minimization \ref{InnerMinAbstract} in a manner analogous to the optimization problem \ref{TRPO_abs}, namely as 
\begin{align}\label{SAM_TRPO_abs}
\begin{split}
    \minimize_{\tilde{\pi}} ~&  \ALoss{\pi_0}(\tilde{\pi})\\
    \text{subject to}~ & \DKLmax(\pi_0,\tilde{\pi})\leq \deltaSAM 
\end{split}
\end{align}
for some trust region constraint $\deltaSAM\geq 0$. We therefore estimate the solution to the inner minimization with the policy $\tilde{\pi}=\pi_{\theta_0+\epsilonSAM}$ where the perturbation $\epsilonSAM=U_{\Fisher{\theta_0}}(\textcolor{red}{-}\nabla_\theta \ALoss{\pi_0}(\theta) \vert_{\theta=\textcolor{red}{\theta_0}}, \deltaSAM)$ is the solution to the optimization problem~\ref{TRPO} where $\Fisher{\theta_0}$ is the Fisher information matrix of our policy parametrization evaluated at $\theta_0$.

Next we proceed to update $\pi_0$ based on the direction provided by the gradient of $\ALoss{\pi_0}$ at our found perturbed parameter $\theta_0+\epsilonSAM$. This step involves solving the maximization problem \ref{TRPO}, where the gradient $\nabla_\theta \ALoss{\pi_0}(\theta)$ is now evaluated at $\theta_0+\epsilonSAM$. This results in a parameter update given by $\epsilonUp=U_{\Fisher{\theta_0}}(\nabla_\theta \ALoss{\pi_0}(\theta) \vert_{\theta=\textcolor{black}{\theta_0+\epsilonSAM}}, \deltaUp)$ where $\deltaUp\geq 0$ is the trust region constraint. The pseudo-code for computing the \MethodName{} gradients is given in Algorithm \ref{SHAPO}. 


\begin{algorithm}[t]
    \caption{\MethodName{}$(\theta,\Obj{},F,\deltaSAM)$}
    \begin{algorithmic}[1]
        \REQUIRE %Policy parametrization $\pi_\theta$,
        parameter $\theta$,
        objective function $\Obj{}$, Fisher matrix $F$, constraint $\deltaSAM$      
        % \STATE Given the SAM constraint $\deltaSAM$ and the optimization objective $\Obj{\pi_\theta}$
        \STATE Compute the gradient at $\theta$: $ g \gets \nabla_\theta \Obj{}(\theta)\vert_{\theta} $
        % \STATE Compute Fisher information matrix: $ F \gets \nabla_\theta \nabla_\theta L_{\pi_\theta}(\theta) $
        \STATE Compute the perturbation: $\boldsymbol{\epsilonSAM}=U_F(\boldsymbol{-}g,\deltaSAM)$%$ \epsilon_{\text{SAM}} \gets F^{-1} g $
        \STATE Compute the gradient at perturbed parameter: $\boldsymbol{\tilde{g}} \gets  \nabla_\theta \Obj{} (\theta) \vert_{\theta + \boldsymbol{\epsilonSAM}} $
        \STATE Return \MethodName{} gradient $\boldsymbol{\tilde{g}}$
    \end{algorithmic}
    \label{SHAPO}
\end{algorithm}

% We observe that selecting an isotropic Euclidean neighborhood in parameter space for $N(\pi_0)$ poses some issues. A small distance in parameter space ($\Vert \theta-\theta_0\Vert_2<\rho$) does not necessarily imply that $\pi_\theta$ is similar to $\pi_0$ in the sense of $\DKLmax$. In this case, $L_{\pi_0(\theta)}<0$ does not ensure that $\ERLag{\lambda}{\pi_\theta}<\ERLag{\lambda}{\pi_0}$. 



% Similarly, to learn a policy $\pi$ that maximizes the risk-aware objective 
% $$
% \min_{\tilde{\pi}\in N(\pi_0)}L_{\pi_0}({\tilde{\pi}}) 
% $$
% % $$
% % \mathcal{R}_{\rho_R}(\tilde{\pi}) = \min_{\DKL{\pi}(\tilde{\pi},\pi)\leq \delta_R}\ERLag{\lambda}{\tilde{\pi}} 
% % $$ 
% or some constant $\delta_R$, we propose to proceed to follow the following local update step. First, with current policy $\pi_0$, we solve the minimization problem corresponding to \ref{TRPO}:
% \begin{align}\label{TRPO_SAM} \begin{split}   \textcolor{red}{\minimize_{\theta}} ~&  \langle \nabla_\theta L_{\pi_0}(\theta) \vert_{\theta=\textcolor{red}{\theta_0}}, (\theta - \theta_0)\rangle \\ 
%     \text{subject to}~ & \frac{1}{2} (\theta - \theta_0)^T A(\theta_0) (\theta - \theta_0)\leq \delta_R 
%     \end{split}
% \end{align}
% By finding the solution $\tilde{\theta}$ of this problem, we aim to find a policy $\pi_{\tilde{\theta}}$ that is close to $\pi_{\theta_0}$ (in the expected KL sense) but effectively performs worse  $\ERLag{\lambda}{\pi_{\tilde{\theta}}}\leq \ERLag{\lambda}{\pi_{\theta_0}}$. 

% Next we solve the maximization problem \ref{TRPO} where the gradient $\nabla_\theta L_{\pi_0}(\theta)$ is now computed at $\tilde{\theta}$:

% \begin{align}\label{TRPO_SAM2} \begin{split}   \textcolor{teal}{\maximize_{\theta}} ~&  \langle \nabla_\theta L_{\pi_0}(\theta) \vert_{\theta=\textcolor{teal}{\tilde{\theta}}}, (\theta - \theta_0)\rangle \\ 
%     \text{subject to}~ & \frac{1}{2} (\theta - \theta_0)^T A(\theta_0) (\theta - \theta_0)\leq \delta 
%     \end{split}
% \end{align}
% The solution $\theta_\text{new}$ of this problem parametrizes the new policy.


\subsection{Reinterpreting Fisher SAM as Pessimism in Face of Epistemic Uncertainty}
\label{sec:sam_risk}

In effect, our proposed approach differs from classical local optimization techniques in that the update of the current parameter $\theta_0$ is guided by the gradient evaluated at $\theta_0+\epsilonSAM$ instead of $\theta_0$. We now provide a different perspective on the perturbation $\epsilonSAM$, arising from a pessimistic viewpoint in the context of epistemic uncertainty.


We propose to model the uncertainty about the parameter $\theta_0$, which defines the current policy $\pi_0=\pi_{\theta_0}$ using a multivariate normal distribution $Q(\theta)=\mathcal{N}(\theta_0, \Sigma)$ with mean $\theta_0$ and covariance matrix $\Sigma=\frac{1}{n}\Fisher{}^{-1}$ where $\Fisher{}^{-1}$ denotes the inverse of the Fisher Information Matrix $\Fisher{}=\Fisher{\theta_0}$ evaluated at $\theta_0$. 
%\revision{For the purpose of our analysis, we denote by $n$ as some ideal measure of the effective sample size used to estimate the parameter $\theta_0$ of the current policy.}
%In our analysis, $n$ denotes the number of interactions or episodes with the environment, thereby highlighting the influence of sample size on the estimation of the parameter $\theta$ that defines the policy $\pi_\theta$.
The choice to model epistemic uncertainty this way is motivated by the asymptotic properties established by the Bernstein--von Mises Theorem \citep{van1998asymptotic} \revision{where $n$ represents the number of independent samples used to estimate the parameters of the model. However, it should be noted that in the case of RL this not simple to compute due to the correlation of samples, as we will elaborate on in Section \ref{subsec:practical}}. This approach captures the intuitive notion that as we gather more data, our uncertainty about the parameter decreases, and the distribution of our estimates becomes more concentrated around the true value. This choice not only aligns with theoretical foundations but also offers a practical starting point for exploring the implications of epistemic uncertainty in the context of policy optimization.

We observe that this uncertainty about the current parameter $\theta_0$ translates into an uncertainty about the expected return $\ERLag{\lambda}{\pi_{\theta}}$ of our current policy, which we can estimate as
$$\ERLag{\lambda}{\pi_{\theta}}\approx \ERLag{\lambda}{\pi_{\theta_0}}+ \ALoss{\pi_0}(\theta)$$ when $\pi_\theta$ is close to $\pi_0$ in distribution.
% This allows to view the random variable $L_{\pi_0}(\theta)$, $\theta\sim Q(\theta)$ as the deviation of expected return. 
Writing $g=\nabla_\theta \ALoss{\pi_\theta}(\theta)\vert_{\theta=\theta_0}$ and assuming a first-order approximation $\ALoss{\pi_0}(\theta+\epsilon)=\epsilon^T g$ around $\theta_0$, the deviation of expected return is given by $Y=\ALoss{\pi_0}(\theta), \theta\sim\mathcal{N}(\theta_0, \frac{1}{n}\Fisher{}^{-1})$ that follows a normal distribution $\mathcal{N}(0,\sigma^2)$ with variance $\sigma^2=\frac{1}{n}g^T \Fisher{}^{-1}g$. 

%While $L_{\pi_0}(\theta_0)=0$ is the mean of this distribution, parameters such that $L_{\pi_0}(\theta)$ fall at, for example, at the $5\th$ percentile of the distribution $Z$ represents a more nuanced view of the distribution, emphasizing that while the mean may suggest a certain level of performance, there are credible scenarios where performance could be significantly lower.

While $\ALoss{\pi_0}(\theta_0) = 0$ represents the mean of this distribution, parameters for which $\ALoss{\pi_0}(\theta)$ falls at, for instance, the 5th percentile of the distribution $Y$ provide a more nuanced perspective on the current expected return. This highlights that, although the mean may indicate a certain level of performance, there are credible scenarios in which performance could be significantly lower. Therefore, adopting a pessimistic standpoint, it is justified to prioritize improving a more conservative expected return when updating $\theta_0$. We demonstrate that evaluating the gradient at $\theta_0 + \epsilonSAM$ to inform the update of $\theta_0$ can be interpreted as optimizing an estimate of the expected return that is pessimistic in face of the parameter uncertainty.

For $\alpha \in (0, \frac{1}{2})$, let $y_\alpha$ denote the $\alpha$-quantile of the random variable $Y$, and $z_\alpha$ denote the $\alpha$-quantile of the normal distribution $\mathcal{N}(0,1)$. %which represents the deviation in expected return due to parameter uncertainty. 
Note that under our first-order approximation of $\ALoss{\pi_0}$ the condition $\ALoss{\pi_0}(\theta_0+\epsilon)\leq y_\alpha$ corresponds to $\epsilon^Tg\leq y_\alpha$.
The following proposition links this epistemic uncertainty perspective with the parameter perturbation described in the previous section. It is illustrated in Fig.~\ref{fig:DualFisher}.

\begin{proposition}\label{prop:SHAPOdual}
    Let $Q(\theta)=\mathcal{N}(\theta_0, \frac{1}{n}\Fisher{}^{-1})$. For every $\alpha\in(0,\frac{1}{2})$, the solution $\epsilon_\alpha$ to the optimization problem
    \begin{align}\label{Epistemic_eps}
\begin{split}
    \maximize_{\epsilon} ~&  \log Q(\theta_0+\epsilon)\\
        \text{subject to}~ & \epsilon^Tg \leq y_\alpha %\ALoss{\pi_0}(\theta_0+\epsilon) \leq y_\alpha
    % \text{subject to}~ & P_Q(\{\theta| L_{\pi_0}(\theta)\leq L_{\pi_0}(\theta_0+\epsilon))\leq \alpha
\end{split}
\end{align}
coincides with the adjustment we make in \MethodName{} for the trust constraint $\deltaSAM=\frac{z_\alpha^2}{2n}$, namely $\epsilon_\alpha= U_{\Fisher{}}(-g,\frac{z_\alpha^2}{2n})$.% for $\deltaSAM=\frac{z_\alpha^2}{n}$,  . 
    % coincides with $\epsilonSAM= U_{\theta_0}(g,\deltaSAM)$ for $\deltaSAM=z_\alpha\frac{1}{\sqrt{n}}\Vert g\Vert_{\Fisher{}^{-1}}$ where $z_\alpha$ is the quantile of $\alpha$ for $\mathcal{N}(0,1)$.
\end{proposition}
Intuitively, this result states that the adjusted parameter $\theta_0 + \epsilonSAM$ considered in \MethodName{} can be viewed as the most likely parameter under the parameter distribution $Q(\theta)$ that falls in the lower tail at the $\alpha$-quantile.
% Intuitively, this result states that the most likely parameter in the lower tail at the $\alpha$-quantile corresponds precisely to the parameter $\theta_0 + \epsilonSAM$, where $\deltaSAM = \frac{y_\alpha^2}{2n}$.
 Our approach \MethodName{}, which updates the current policy \(\pi_0\) by using the gradient $\tilde{g}$ calculated at this adjusted parameter, can therefore be understood as promoting an enhancement of \(\pi_0\) in a worst-case or pessimistic scenario, considering the existing epistemic uncertainty surrounding \(\pi_0\). 
\revision{By applying \MethodName{} with a $\deltaSAM>0$ to update the actor, we are therefore effectively enforcing pessimism in face of epistemic uncertainty about our current policy.}

% Our approach SHAPO 
% Updating the current policy \(\pi_0\) by using the gradient $\tilde{g}$ calculated at the adjusted parameter can therefore be understood as promoting an enhancement of \(\pi_0\) in a worst-case or pessimistic scenario, considering the existing epistemic uncertainty surrounding \(\pi_0\).
%Therefore guiding the update of the current policy $\pi_0$ using the gradient evaluated at this adjusted parameter can be viewed as promoting an update that aims at improving $\pi_0$ in a worst case or pessimistic scenario in face of epistemic uncertainty. 

%The most likely parameter that evaluates to at most the 5th percentile highlights scenarios where the expected return is particularly low. This focus is crucial for understanding the boundaries of performance and recognizing the potential risks associated with the policy. The most likely parameter within this tail is not just a random selection; it represents a credible outcome based on the observed data, making it a valuable point of reference for updating the policy.
Furthermore, by establishing the relationship \(\deltaSAM = \frac{z_\alpha^2}{2n}\), this proposition allows us to interpret the constraint \(\deltaSAM\) as a measure of confidence in the expected return of the current policy in the presence of epistemic uncertainty. More details and proof in Appendix \ref{sec:fischer}.

\begin{figure}[t]
    \centering
    \includegraphics[height=2cm]{iclr2026/figs/Main1.png}\qquad     \includegraphics[height=2cm]{iclr2026/figs/Main2.png}
    \qquad     \includegraphics[height=2cm]{iclr2026/figs/Main3.png}
    % \includegraphics[height=2cm]{iclr2026/figs/FisherDual.png} \qquad \includegraphics[height=2cm]{iclr2026/figs/MainUp.png}
    \caption{\small{
    \MethodName{} directs the policy update using the gradient \(\tilde{g}\) at an adjusted parameter (Right). Two perspectives on this adjustment are illustrated: (Left) The adjustment aims to minimize the expected return while staying within the trust region defined by \(\deltaSAM\). (Middle) Parameter uncertainty translates to uncertainty in the expected return, resulting in a maximum likelihood adjustment that remains below the \(\alpha\)-quantile \(y_\alpha\).
    % \MethodName{} guides the policy update using the gradient $\tilde{g}$ at an adjusted parameter (Right). Two perspectives on the parameter adjustment of \MethodName{}. Left: Parameter uncertainty translates to uncertainty about the expected return of the current policy, leading to an adjustment with maximum likelihood while representing to an expected return below the $\alpha$-quantile $y_\alpha$. Middle: The adjustment is framed so as to minimize the expected return while staying in the trust region specified by $\deltaSAM$. 
    }}
    \label{fig:DualFisher}
\end{figure}



% Say that now the geometric $\deltaSAM$ can be interpreted as coming from a confidence level.

%Move to appendix
%

% \alert{
% The relation $\deltaSAM=\frac{z_\alpha^2}{n}$  provides an interesting perspective on the trust constraint for minimization in \MethodName{}. It expresses the bound in terms of the $\alpha$-quantile of the normal distribution $\mathcal{N}(0,1)$ and $n$ that represents the sample size used for estimating $\theta_0$. For a given sample size $n$, choosing a confidence level, say $5$th percentile, leads to value for $\deltaSAM$. This suggests choosing an initial $\deltaSAM$ by choosing a confidence level $z_\alpha$ and then decrease the $\deltaSAM$ linearly as our actor is exposed to more experience.  
% }


% \alert{ 
% Try to explain that $\nabla_\theta \ALoss{\pi_0}(\theta+\epsilonSAM)\vert_{\theta_0}=\nabla_\theta \ALoss{\pi_0}(\theta)\vert_{\theta_0+\epsilonSAM}$ coincides with the gradient of the mean parameter of $Q(\theta)=N(\theta_0,\Sigma)$ for the objective $\ALoss{\pi_0}(\theta+\epsilonSAM)$  ?
% }

% \alert{
% The expected advantage $\E_{\theta\sim Q}\ALoss{\pi_0}(\theta)$ coincides with $\ALoss{\pi_0}(\theta_0)=0$ under our first-order approximation of $\ALoss{\pi_0}$. Hence maximizing the expected advantage under $Q$ falls back to maximizing $\ALoss{\pi_0}(\theta)$. However, maximizing instead the advantage at the most likely parameter in the lower tail at the $\alpha$-quantile amounts to maximize $\ALoss{\pi_0}(\theta_0+\epsilon_\alpha)=\ALoss{\pi_0}(\theta_0+\epsilonSAM)$, which leads to guiding the update of $\theta_0$ in the direction of $\nabla_\theta \ALoss{\pi_0}(\theta+\epsilonSAM)\vert_{\theta_0}=\nabla_\theta \ALoss{\pi_0}(\theta)\vert_{\theta_0+\epsilonSAM}$. 
% }



%that for, say $\alpha=0.05$, there is a bound $\delta(\alpha)$ such that the corresponding perturbed parameter $\theta_0+\epsilonSAM$ coincides with the most likely parameter under $Q(\theta)$ such that $5\%$ of the parameters get a lower value.  




% \section{Fisher--SAM as a Bayesian VaR/CVaR Objective}
% \label{subsec:fsam_bayes_cvar}

% We work around a reference policy $\pi_{\theta_0}$ and its TRPO surrogate
% \begin{equation}
% \mathcal{L}_{\theta_0}(\theta)
% = \mathbb{E}_{s\sim d^{\pi_{\theta_0}},\,a\sim \pi_{\theta_0}}
% \!\Big[\tfrac{\pi_\theta(a\mid s)}{\pi_{\theta_0}(a\mid s)}\,A_{\pi_{\theta_0}}(s,a)\Big].
% \tag{S1}
% \end{equation}
% Let $F_0$ denote the (average) Fisher information at $\theta_0$:
% \begin{equation}
% F_0
% := \mathbb{E}_{s\sim d^{\pi_{\theta_0}},\,a\sim \pi_{\theta_0}}
% \!\big[\nabla_\theta\log \pi_{\theta_0}(a\mid s)\,\nabla_\theta\log \pi_{\theta_0}(a\mid s)^\top\big].
% \tag{S2}
% \end{equation}
% Define the Fisher--SAM (FSAM) robust surrogate (for maximization) via an inner adversary constrained in the Fisher geometry:
% \begin{equation}
% \mathcal{R}_\rho(\theta)
% := \min_{\Delta:\ \Delta^\top F_0 \Delta \le \rho^2}\ \mathcal{L}_{\theta_0}(\theta+\Delta).
% \label{S3}
% \end{equation}

% \paragraph{Local Bayesian model and assumptions.}
% We adopt a local Bayesian view near $\theta_0$: the parameter is random as
% \begin{equation}
% \theta \sim \mathcal{N}(\mu,\Sigma), \qquad \mu \approx \theta_0,
% \label{A1}
% \end{equation}
% and we linearize the surrogate at $\mu$:
% \begin{equation}
% \mathcal{L}_{\theta_0}(\theta)\ \approx\
% \mathcal{L}_{\theta_0}(\mu) + g_0^\top(\theta-\mu),\qquad
% g_0 := \nabla_\theta \mathcal{L}_{\theta_0}(\theta)\big|_{\theta=\mu}.
% \label{A2}
% \end{equation}
% To connect the Fisher metric with posterior uncertainty we use one of two standard identifications:
% \begin{align}
% \text{(Posterior-precision metric)}\quad &\Sigma^{-1}\ \text{is known/estimated, and we use it directly;} \label{A3a}\\
% \text{(Average-Fisher metric)}\quad &\Sigma^{-1}\ \approx\ n\,F_0\ \ \text{(Laplace/BvM, flat prior), with effective size } n. \label{A3b}
% \end{align}

% \paragraph{Inner FSAM solution as a Fisher-norm penalty.}
% \begin{lemma}[Support function of a Fisher ellipsoid]
% \label{lem:fisher_support}
% For any differentiable $f$ and fixed $\theta$, with $g(\theta):=\nabla_\theta f(\theta)$ and $F_0\succ 0$,
% \[
% \max_{\Delta:\ \Delta^\top F_0\Delta\le \rho^2} g(\theta)^\top \Delta
% = \rho\,\|g(\theta)\|_{F_0^{-1}},
% \qquad
% \text{where }\ \|v\|_{F_0^{-1}} := \sqrt{v^\top F_0^{-1}v}.
% \]
% \end{lemma}
% \begin{proof}
% Let $u=F_0^{1/2}\Delta$. The constraint is $\|u\|_2\le \rho$ and
% $g^\top\Delta=(F_0^{-1/2}g)^\top u \le \|F_0^{-1/2}g\|_2\,\|u\|_2$ by Cauchy--Schwarz.
% Equality holds for $u$ aligned with $F_0^{-1/2}g$.
% \end{proof}

% Applying Lemma~\ref{lem:fisher_support} to \eqref{S3} with the first-order expansion
% $\mathcal{L}_{\theta_0}(\theta+\Delta)\approx \mathcal{L}_{\theta_0}(\theta)+\nabla \mathcal{L}_{\theta_0}(\theta)^\top \Delta$
% gives the familiar FSAM penalty:
% \begin{equation}
% \mathcal{R}_\rho(\theta)
% = \mathcal{L}_{\theta_0}(\theta)\ -\ \rho\,\|\nabla_\theta \mathcal{L}_{\theta_0}(\theta)\|_{F_0^{-1}}
% \ +\ o(\rho).
% \label{S4}
% \end{equation}

% \paragraph{Distribution of the linearized Bayesian surrogate.}
% Under \eqref{A1}--\eqref{A2}, the random surrogate
% \begin{equation}
% Z := \mathcal{L}_{\theta_0}(\theta)\ \approx\ \mathcal{L}_{\theta_0}(\mu)+g_0^\top(\theta-\mu)
% \end{equation}
% is Gaussian:
% \begin{equation}
% Z \sim \mathcal{N}\!\big(\mathcal{L}_{\theta_0}(\mu),\,\sigma^2\big),
% \qquad
% \sigma := \sqrt{g_0^\top \Sigma g_0}.
% \label{S5}
% \end{equation}
% In particular, under \eqref{A3b} we have $\sigma=\|g_0\|_{F_0^{-1}}/\sqrt{n}$, whereas under \eqref{A3a} we simply keep $\sigma=\sqrt{g_0^\top\Sigma g_0}$.

% \paragraph{Equivalence to VaR and CVaR.}
% Let $\Phi$ and $\phi$ be the CDF/PDF of $\mathcal{N}(0,1)$ and $z_\alpha:=\Phi^{-1}(\alpha)$ for $\alpha\in(0,1)$ (so $z_\alpha<0$ for lower tails).
% The lower-tail risk measures of $Z$ are
% \begin{align}
% \mathrm{VaR}_\alpha[Z] &= \mathcal{L}_{\theta_0}(\mu) + \sigma\,z_\alpha
% = \mathcal{L}_{\theta_0}(\mu) - |z_\alpha|\,\sigma, \label{S6}\\
% \mathrm{CVaR}_\alpha[Z] &= \mathbb{E}[Z\mid Z\le \mathrm{VaR}_\alpha(Z)]
% = \mathcal{L}_{\theta_0}(\mu) - \frac{\phi(z_\alpha)}{\alpha}\,\sigma.
% \label{S7}
% \end{align}

% \begin{theorem}[FSAM equals Bayesian VaR/CVaR under the local model]
% \label{thm:fsam_var_cvar}
% Evaluate \eqref{S4} at $\theta=\mu$.
% \begin{enumerate}
% \item (Posterior-precision metric \eqref{A3a}) With $\sigma=\sqrt{g_0^\top\Sigma g_0}$,
% \[
% \mathcal{R}_\rho(\mu)
% = \mathcal{L}_{\theta_0}(\mu) - \rho\,\|g_0\|_{F_0^{-1}}
% \overset{\text{\tiny (A3a)}}{=}\ \mathcal{L}_{\theta_0}(\mu) - \rho\,\sigma
% \]
% so choosing $\rho=|z_\alpha|$ yields $\mathcal{R}_\rho(\mu)=\mathrm{VaR}_\alpha[Z]$, and choosing $\rho=\phi(z_\alpha)/\alpha$ yields $\mathcal{R}_\rho(\mu)=\mathrm{CVaR}_\alpha[Z]$.
% \item (Average-Fisher metric \eqref{A3b}) With $\sigma=\|g_0\|_{F_0^{-1}}/\sqrt{n}$,
% \[
% \mathcal{R}_\rho(\mu)=\mathcal{L}_{\theta_0}(\mu)-\rho\,\|g_0\|_{F_0^{-1}}
% = \mathcal{L}_{\theta_0}(\mu) - \big(\rho\sqrt{n}\big)\,\sigma,
% \]
% so matching VaR/CVaR requires
% \[
% \rho \ =\ \frac{|z_\alpha|}{\sqrt{n}}
% \quad \text{(VaR)},\qquad
% \rho \ =\ \frac{\phi(z_\alpha)}{\alpha\,\sqrt{n}}
% \quad \text{(CVaR)}.
% \]
% \end{enumerate}
% \end{theorem}
% \begin{proof}
% For (1), combine \eqref{S4} at $\theta=\mu$ with $\|g_0\|_{F_0^{-1}}=\sigma$ under \eqref{A3a} and match coefficients with \eqref{S6}--\eqref{S7}.
% For (2), use $\sigma=\|g_0\|_{F_0^{-1}}/\sqrt{n}$ under \eqref{A3b} and again match coefficients.
% \end{proof}

% \paragraph{Credible-ellipsoid calibration (multivariate).}
% Let $\mathcal{C}_\alpha:=\{\theta:\ (\theta-\mu)^\top F_0(\theta-\mu)\le \chi^2_{d,\,1-\alpha}\}$.
% Under \eqref{A3b}, $\mathbb{P}(\theta\in \mathcal{C}_\alpha)\approx 1-\alpha$ and
% \[
% \min_{\theta\in \mathcal{C}_\alpha}\ \mathcal{L}_{\theta_0}(\theta)
% \ \approx\ \mathcal{L}_{\theta_0}(\mu) - \sqrt{\chi^2_{d,\,1-\alpha}}\ \|g_0\|_{F_0^{-1}}/\sqrt{n},
% \]
% which is a conservative (multivariate) lower credible bound consistent with Theorem~\ref{thm:fsam_var_cvar}.

% \paragraph{Scope and caveats.}
% The equivalence holds under the local linearization \eqref{A2} and the Gaussian posterior approximation \eqref{A1} with either \eqref{A3a} or \eqref{A3b}. In misspecified or singular regimes, $\Sigma^{-1}$ may follow a (Bayesian) sandwich form; practically one can (i) damp $F_0$ by $\lambda I$ and (ii) treat $n$ in \eqref{A3b} as an effective on-policy sample size. Importantly, the geometry remains TRPO-consistent: the inner FSAM set and the trust region both live in the Fisher/KL metric, and $\rho$ cleanly controls risk aversion (VaR/CVaR level) measured in posterior standard deviations.

\input{iclr2026/sections/gaussian_policy_analysis}

% \subsection{SAM on critic}
\revision{
\subsection{\MethodName{} for on-policy RL algorithms}
\label{subsec:practical}
}
\begin{revisionblock}
As presented in this section, Sharpness Aware Policy Optimization (\MethodName{}) modifies the TRPO algorithm with a Lagrange objective and pseudo-code is provided in Algorithm~\ref{SAM-TRPO}. We abstract this modification in Algorithm~\ref{SHAPO}: this code returns a parameter direction $\tilde{g}$ for updating the current policy $\pi_\theta$ based on the objective function $L$, the Fisher matrix $F$ of the policy parametrization and constraint bound $\deltaSAM$. Formulated this way, our method can be applied to most online policy RL algorithms and we provide pseudo-code in Appendix~\ref{sec:pseudo} for CRPO and CPO. 
\end{revisionblock}
% \revision{We provide pseudo-code for \MethodName{} in Algorithm~\ref{SHAPO}. Formulated this way, our method can be applied to most online policy RL algorithms. It returns a parameter direction $\tilde{g}$ for updating the current policy $\pi_\theta$ based on the objective function, the Fisher matrix of the policy parametrization and constraint bound $\deltaSAM$. This function effectively abstracts lines $4-7$ of Algorithm~\ref{SAM-TRPO} and allows us to present how our method applies to other algorithms. Our method applies to any on policy RL algorithms, we provide details in Appendix A.}


% \subsection{Scheduling Pessimism}
\begin{revisionblock}

While Proposition~\ref{prop:SHAPOdual} links the trust-region constraint $\deltaSAM$ to the percentile $z_\alpha$ of the normal distribution (where $\alpha$ is the level of pessimism in face of uncertainty), the effective sample size $n$ cannot be easily estimated in continuous-control reinforcement learning where data are temporally correlated and only a subset of collected samples provide independent information. Furthermore, due to the complex coupling between the actor and critic, together with the challenges posed by exploration, it is difficult to determine the appropriate level of pessimism (\textit{i.e.} the value of $\alpha$) to adopt at each stage of the training. 

In this context, adopting a constant value of $\deltaSAM$ during training and treating this value as tunable hyperparameter allows us to directly control the desired safety--efficiency tradeoff without relying on uncertain estimates of $n$. This makes the constant-$\deltaSAM$ strategy both simple and effective, offering a stable mechanism for regulating pessimism throughout training. We further discuss this approach and other options to schedule the level of pessimism in Subsection~\ref{subsec:ablation} and in Appendix~\ref{sec:alpha_delta}. 

\end{revisionblock}

\begin{figure}[t]
    \centering
    \vspace{-0.5cm}
    \includegraphics[width=\linewidth]{iclr2026/figs/results_main.png}
    \vspace{-2em}
        \caption{\small{Performance of \MethodName{} on four different tasks across four different baselines over $5$ training seeds. We report Cost Rate (Total Cost / Total Env Steps) for Safety Gym environments after training for $10M$ environment steps and Total Cost for MuJoCo environments after $5M$ environment steps. \MethodName{} (shown with a star) significantly improves the performance of the baseline algorithms (shown with a circle) on both safety and efficiency thus improving the safe exploration capabilities of the baseline algorithms. \revision{Width and height of the ellipses represent the standard error over 5 seeds. %in both the $x$-direction (cost rate or total cost) and the $y$-direction (return).
        } }}
        
    \label{fig:results_main}
    % \vspace{-0.3cm}
\end{figure}


\begin{figure}[t] % 'h' for placing figures near here in the text
  % \vspace{-0.5cm}

  \centering
  \vspace{-1em}
  \begin{minipage}{0.49\textwidth} % First figure, takes up 48% of the text width
    \centering
    \includegraphics[width=\linewidth]{iclr2026/figs/lambda_pareto_pidlag.png}
    \vspace{-2em}
    \caption{\small{Results for different values of initial lambda ($\lambda_{init}$) for \textit{PIDLag} algorithm with and without \MethodName{}. We can see that \MethodName{} improves upon the Vanilla \textit{PIDLag} for all configurations.}}
    \label{fig:lambda_pareto}
  \end{minipage}
  \hfill
  \begin{minipage}{0.49\textwidth} % Second figure, also takes up 48% of the text width
    \centering
    \includegraphics[width=\linewidth]{iclr2026/figs/shapo_epcost_tail.png}
    \vspace{-2em}
    \caption{\small{\MethodName{} results in policies with episodic cost distributions with smaller tails (80th percentile and 95th percentile)  crucially for safe exploration during the learning phase.}}
    \label{fig:epcost_tail}
  \end{minipage}
  \vspace{-0.5cm}

\end{figure}
%% Old version 


% Since determining the optimal value for δDown at each update step poses a significant challenge, we
% opted for a simple and practical approach: considering the value of δDown as a hyperparameter and
% constantly use the same value for each update step across training. While Proposition 2 connects
% the trust region constraint δDown to the percentile zα of the normal distribution, correctly estimating
% the effective number of samples n that have been used for optimizing the actor at a given step of the
% learning algorithm is not straightforward. Moreover, considering the complex interplay between the
% actor and the critic, along with the challenges of exploration, it is unclear what level of pessimism
% should be adopted at each step of the learning process in face of the epistemic uncertainty about the
% actor. We discuss the fixed δDown approach and other options to schedule the level of pessimism in
% Subsection 6.1.





% Since determining the optimal value for $\deltaSAM$ at each update step poses a significant challenge, we opted for a simple and practical approach: considering the value of $\deltaSAM$ as a hyperparameter and constantly use the same value for each update step across training.
% While Proposition~\ref{prop:SHAPOdual} connects the trust region constraint $\deltaSAM$ to the percentile $z_\alpha$ of the normal distribution, correctly estimating the effective number of samples $n$ that have been used for optimizing the actor at a given step of the learning algorithm is not straightforward. Moreover, considering the complex interplay between the actor and the critic, along with the challenges of exploration, it is unclear what level of pessimism should be adopted at each step of the learning process in face of the epistemic uncertainty about the actor. We discuss the fixed $\deltaSAM$ approach and other options to schedule the level of pessimism in Subsection~\ref{subsec:ablation}. 
% While Proposition 2 provides a valuable perspective on our \MethodName{} method, determining the appropriate value for $\deltaSAM$ (or $\alpha$) at each update step poses a significant challenge. Indeed, scheduling the appropriate amount of pessimism for updating the actor is a difficult problem. Say something about RL exploration etc.  Firstly, while the relationship \(\deltaSAM = \frac{z_\alpha^2}{2n}\) connects the trust region constraint $\deltaSAM$ to the percentile $z_\alpha$ of the normal distribution, accurately estimating the sample size $n$ used for optimizing the actor at a given step of the learning algorithm is not straightforward. Secondly, considering the complex interplay between the actor and the critic, along with the challenges of exploration, it remains uncertain what level of pessimism we should adopt in response to the epistemic uncertainty of the actor at each step of the learning process. In this context, in our implementation we opted for a simple and practical approach: considering the value of $\deltaSAM$ as a hyperparameter and constantly use the same value for each update step across training. However, we also investigated a different approach treating $\alpha$ as hyperparameter at each step $t$ estimate the sample size by the number $n_t$ of state-action pairs collected so far by our agent.
%a) Talk about $n$ i.e. the effective sample size here. b) Describe what happens when delta is kept fixed and what it means to decay delta which is to fix alpha. c) Explain why fixing delta might be desirable for safe exploration setting where you don't want your agent to become too conservative.


Finally, in our method, we also incorporate Sharpness Aware Minimization with Euclidean neighborhoods for the critic, as proposed by~\cite{sam} for a supervised learning task. By considering the sharpness of the loss landscape during the training of the critic, we aim to focus on flatter regions that yield more stable value function approximations. %This approach helps reduce overfitting and enhances the critic's ability to generalize across various states and actions, resulting in more reliable value estimates for improved decision-making in the reinforcement learning framework.


